Global Convergence to Nash Equilibrium in Nonconvex General-Sum Games under the $n$-Sided PL Condition

We consider the problem of finding a Nash equilibrium (NE) in a general-sum game, where player $i$'s objective is $f_i(x)=f_i(x_1,...,x_n)$, with $x_j\in\mathbb{R}^{d_j}$ denoting the strategy variables of player $j$. Our focus is on investigating first-order gradient-based algorithms and their variations, such as the block coordinate descent (BCD) algorithm, for tackling this problem. We introduce a set of conditions, called the $n$-sided PL condition, which extends the well-established gradient dominance condition a.k.a Polyak-{\L}ojasiewicz (PL) condition and the concept of multi-convexity. This condition, satisfied by various classes of non-convex functions, allows us to analyze the convergence of various gradient descent (GD) algorithms. Moreover, our study delves into scenarios where the standard gradient descent methods fail to converge to NE. In such cases, we propose adapted variants of GD that converge towards NE and analyze their convergence rates. Finally, we evaluate the performance of the proposed algorithms through several experiments.

==> AAMAS-2026-Formatting-Instructions-CCBY/limitations.tex <==
\section{Limitations}

==> AAMAS-2026-Formatting-Instructions-CCBY/rebuttal.tex <==
\textbf{Reviewer qtGL}

I enjoyed reading the paper, and it was well written. However, I do not believe it meets AAMAS's requirements for publication. Per AAMAS's instructions on supplementary material: "Any information that is essential for understanding or evaluating your paper must be included in the paper itself. For example, it is not recommended to relegate most of the proofs of your theoretical results to the supplementary material". In the case of this paper, all information that is essential for understanding the paper is in the 16-page supplementary material. Notably, since the supplementary material is not published, no results in this paper are verifiable to the general audience. As a result, this paper seems outside of AAMAS's scope, and I regretfully recommend rejection.

{\color{blue} 

We sincerely thank the reviewer for taking the time to read and evaluate our paper, and we are glad that you found it well-written and enjoyable to read. We would like to respectfully clarify that due to the 8-page limit imposed by AAMAS, we followed a common practice in this venue of placing detailed proofs and technical derivations in the supplementary material, while presenting all main results, intuitions, and key derivations in the main text. For reference, several papers previously published in AAMAS have followed the same approach, placing lengthy proofs in the supplementary material. 
These examples demonstrate that including detailed proofs in the supplementary material is consistent with AAMAS practices, and the main paper remains verifiable and understandable to the audience.

We hope this clarifies our rationale for structuring the paper in this manner and that our work will be assessed on the basis of its merits and its theoretical contributions to the field of game theory. 

[1] FedRLHF: A Convergence-Guaranteed Federated Framework for Privacy-Preserving and Personalized RLHF, Flint Xiaofeng Fan, Cheston Tan, Yew-Soon Ong, Roger Wattenhofer, Wei Tsang Oo, AAMAS 2025

[2] Provably learning Nash policies in constrained Markov potential games Alatur P, Ramponi G, He N, et al.  AAMAS 2024.


[3] Divide and conquer: Provably unveiling the Pareto front with multi-objective reinforcement learning. Röpke, W., Reymond, M., Mannion, P., Roijers, D. M., Nowé, A.,  Rădulescu, R. AAMAS 2025


}


Some larger questions/comments:

How strong is (6)? I don't work too much in the convex/concave game case and am unsure. In your claim that it isn't restrictive, you show all smooth functions, n-sided PL functions satisfy (6) with $\kappa = \sqrt{3n}L/\mu >=1$. However, Theorem 3.3 requires $\kappa <1$... so it seems there is no reason to expect it to hold for many functions. You claim that (6) is overly restrictive, then give a bound that doesn't at all support the statement... the mathematical statement after (6) actually suggests that (6) is very restrictive.

{\color{blue} 
This is a kin observation by the reviewer. To clarify this, we would like to re-stated the following remarks:

- Firstly, please note that assumption in (6) is a condition required for linear convergence of R-BCD algorithm. When this assumption is not satisfied, we propose two alternative algorithms: IA-RBCD and A-RBCD—to fully solve the problem, each with its corresponding convergence rate.

- Secondly, as it is stated after Theorem 3.3., the introduced bound, $\kappa\leq\sqrt{3n}L/\mu$, is generally greater than $1$. 
However, please note that the main purpose of introducing this bound was to demonstrate that the ratio of the left-hand side to the right-hand side of (6) is bounded, i.e., 
$$
\frac{\sum_{i=1}^n \big\langle \nabla_i G_F(x) - \nabla_i F_{-i}(x), \nabla_i f_i(x) \big\rangle
}{ \sum_{i=1}^n \|\nabla_i f_i(x)\|^2}\leq \sqrt{3n}\tfrac{L}{\mu}<\infty.
$$
Thus, the inequality in (6) is well-defined for all smooth n-sided PL functions. 
However, this inequality only provides an upper bound, which means that for some functions the above ratio can be less than one, while for others it can be greater than one. In Theorem 3.3, we showed that for functions where this ratio is strictly less than one, the R-BCD algorithm converges linearly. As mentioned after the theorem, there are functions, for example, those depicted in Figures 2 and 3, for which the ratio exceeds one.
%However, the purpose of this bound is not to prove $\kappa<1$ globally. Instead, it shows: for any smooth n-sided PL function, the left-hand side of (6) is always bounded by a constant multiple of $\sum_i\|\nabla_i f_i(x)\|^2$, which is stated in the manuscript. The role of this bound is to show that (6) is well-defined for all smooth n-sided PL functions and many functions satisfy (6) with $\kappa < 1$ in regions relevant for convergence.
}



How strong is Definition 3.4? [38] doesn't really indicate much since it is only satisfies for a neighborhood around the optimizer; Theorem 3.5 needs it to hold in general (in less you are waiting on Case 3 to kick in once we are sufficiently close to an equilibrium.

{\color{blue} 

To address this question, note that the $(\theta,\nu)$-PL condition in Definition 3.4 is **not required for convergence**, but it helps to specify the convergence rate. Thus, even without this condition, the algorithms **will provably converge**, as mentioned in Case 3, where it is introduced only as an additional assumption.

Moreover, Definition 3.4 does **not need to hold globally**. To see this, consider the result of Theorem 3.7, which implies that by letting $\gamma\to 1$ and $C\to 0$, we can shrink the region where Cases 1 and 2 do not occur, or equivalently, shrink the region for Case 3 to a **local area around a stationary point**. Therefore, a local $(\theta,\nu)$-PL condition is sufficient to prove the convergence rates presented.


%Firstly, we need to specify that Definition 3.4 is not required for the convergence, but for the convergence rate. Secondly, we still don't require definition 3.4 satisfy globally. We could shrink the area that cases 1 and 2 don't cover by making $\gamma\to 1$ and $C\to 0$. Thus, a local PL condition is mathematically sufficient and no global requirement is imposed. 
}

Minor comment:

Computation of a best response in itself can be a time-consuming action. I did not see where the analysis takes this part into consideration.

{\color{blue} Please note that in Lemma 3.8. and Theorem 3.9., we analyze the number iteration $T'$ to achieve a good approximation of the best response.}

"Note this is not a limiting assumption given that the function is lower bounded". I reread the notation section a few times and could never find this assumption.

Title of D.3 is incorrect. You also have a x* instead of a $x^*$

missing parentheses after the comment on (6) not being restrictive (see Lemma A.3. for a proof that $\mu \leq L$).

Definition 3.4: A function f with ...

Definition 3.4: Is the same PL condition (was it introduced in the same papers that introduced the original definition). When I first read 3.4, I assumed you were proposing the modification, but the next line suggests this isn't the case.

{\color{blue} Please note that the ($\theta$,$\nu$)-PL condition is an extension of the PL condition in equation (2), i.e. $\theta=2$ and $\nu=\mu$. In this paper, our proposed $n$-sided PL condition is an extension of the PL condition, i.e., $n=1$.}

Accessing the gradient $\nabla G_F$ presumably requires additional sampling... fine for most settings, but something for applications where agents might not be able to coordinate to access such info. The authors acknowledge something to this effect by stating it "it can be computed using the gradients at the best responses".
{\color{blue} Thank you for your comments. To run IA-RBCD and A-RBCD, agents need to have access to the info about the best response and communicate with each others. However, we also want to specify that the $n$-sided PL condition is very general, as for every agent, it only requires the PL condition for one block of coordinates. }

The colors used in your graphs are not consistent (e.g., Figure 5 uses green for A-RBCD but Figure 5 uses yellow for A-RBCD).


{\color{blue}
We are grateful for your attention to the minor typos and errors and will ensure that they are all corrected in the final version.
}












\newpage
\textbf{Reviewer 3fjL}

This work defines the notion of n-sided PL, subsequently developing new insights into the structural properties of the according functions, and utilizing them to obtain better ways to guide gradient descent algorithms (here, the observed relation to the sum of best responses appeared most notable to me, and it was nice to see this submission build on a clear, simple, yet key insight).

To achieve this, the authors restrict the setting in additional ways. The introduction of these additional assumptions, justified given the challenging setting, seemed in most parts consequential (however the explanations given for them were sometimes more, sometimes less clear to me). Even under several restrictions (n-sided PL, smoothness, existence of Nash Equilibria etc.), this work still captures a relatively broad class of settings (see experiments section).

W.r.t. previous work, the authors state as a main achievement the applicability to general-sum-games, which was not the case there. This seems like a considerable achievement to me, although I am not too familiar with the according literature.

The general chain of arguments, identifying NE as corresponding to stable points, then using the distance in the sum of objectives/best responses, is intuitive and convincing given assumptions that guarantee the above correspondence. It is also presented in a reasonable fashion and repeatedly accompanied by comparisons to existing work and known concepts. However, the idea at the heart of the achieved results appears naturally restricted to essentially the assumptions made (possibly similar variants), which somewhat limits its potential.

Typos/minor

P2 ‘We show that the convergence to NE and introduce additional local conditions’

p2 ‘requires the computational complexity of the order’

p3 ‘has a local minima, a global minima’

p5 ‘satisfy n-sided mu-PL and satisfies’

p5 The above result further highlight

p7 there is no figure 4a).

p8 ‘are not lower bounded and has strict saddle points’


{\color{blue}
We sincerely thank the reviewer for the thorough and thoughtful evaluation of our work. We are glad that the notion of $n$-sided PL and its structural insights, as well as the relation to the sum of best responses, were found notable and insightful. We also appreciate your recognition of the applicability of our approach to general-sum games.

We acknowledge your comments regarding the clarity of some explanations for the additional assumptions. We will revise the manuscript to make these justifications more precise and accessible. We also appreciate your careful identification of minor typos and errors, and we will ensure that all of these are corrected in the final version.

}


\newpage
\textbf{Reviewer ViM9}

The paper is interesting and well written, achieving a rigorous formal form. Authors clearly define the goal of the paper and present related works well. The most important parts of the paper are Sections 3 and 4, which present different variants of algorithms with convergence analysis and their applications.

The proposed algorithms have been evaluated through several experiments. Their performance and results obtained are deeply discussed in the paper.

I do not have any significant objections related to the paper.

In my opinion, the paper may be considered as a candidate for presentation during the conference.



{\color{blue}
We sincerely thank the reviewer for the positive and encouraging evaluation of our paper. We are glad that the presentation, the formal rigor, and the discussion of our proposed algorithms and their applications were found clear and comprehensive. Your supportive comments reinforce the contribution of our work.
}

==> Algorithm.tex <==
\vspace{-.3cm}
\section{Algorithms and Convergence Analysis}\label{sec:algs}

In this section, we first study the BCD algorithm for finding a stationary point of \eqref{min_problem} under the $n$-sided PL condition. 
Afterward, we propose different variants of BCD algorithms that can provably achieve better convergence rates. 

The BCD algorithm is a coordinate-wise approach that iteratively improves its current estimate by updating a selected block coordinate using the first-order partial derivatives until it converges. 
\vspace{-.3cm}
\begin{algorithm}[H]
\caption{Cyclic Block Coordinate Descent (BCD)}\label{alg:BCD}
\begin{algorithmic}
   \STATE {\bfseries Input:} initial point $x^0=(x_1^0,...,x_n^0)$, learning rates $\{\alpha_i^t\}$
   \FOR{$t=1$ {\bfseries to} $n$}
   \FOR{$i=1$ {\bfseries to} $n$}
   \STATE $x_i^t=x_i^{t-1}-\alpha_{i}^t\nabla_{i}f(x_{1:i-1}^t,x_{i:n}^{t-1})$
   \ENDFOR
   \ENDFOR
  % \STATE {\bfseries Output:} $x^T=(x_1^T,...,x_n^T)$
\end{algorithmic}
\end{algorithm}
\vspace{-.3cm}
It is important to note that BCD algorithms typically utilize the partial gradient evaluated at the latest estimated point to update the selected coordinate. 
Depending on how the coordinates are chosen, various types of BCD algorithms can be devised.
For example, coordinates can be selected uniformly at random, \textit{random BCD}, or in a deterministic cyclic sequence, progressing one after another. 
Algorithm \ref{alg:BCD} presents the \textit{cyclic BCD} algorithm with {learning rates} $\{\alpha_{i}^t\}$. %, where coordinates are cyclically selected one after another. 
Moreover, to update the $i$-th block at the $t$-th iteration, it employs $\nabla_{i}f(x_{1:i-1}^t,x_{i:n}^{t-1})$, where $(x_{1:i-1}^t,x_{i:n}^{t-1})$ denotes the latest estimated point and it is $(x_1^t,...,x_{i-1}^t,x_i^{t-1},...,x_n^{t-1})$.
Next result shows that when the iterates of the BCD, $\{x^t\}$ are bounded, the output converges to the NE set. 
%From \cite{xu2013block}, the convergence to the set of stationary points can be proved. In addition, the equivalence of Nash Equilibrium and the stationary point is proved in \cref{SP_equal_NE}, which indicates the convergence to the Nash Equilibrium.

\begin{theorem}\label{bounded_to_converge}
Under the \cref{derivative_Lip} and \cref{lower-bounded}, if $f(x)$ satisfies $n$-sided PL condition, the iterates $\{x^t\}$ are bounded and the learning rates \textcolor{red}{change to $1/L$ $\alpha_i^t=\alpha\leq\frac{1}{L_c}$}, then $\lim_{t\to+\infty}dist\big(x^t,\mathcal{N}(f)\big)=0$.
\end{theorem}


The above result ensures the convergence of BCD to the NE set, but it does not necessarily indicate whether the output converges to a point within the NE set. 
The convergence to a point within the NE set can be established if further every point in the NE set is isolated, e.g., $f_0$ and $f$ in Figure \ref{fig:example1}. %Formally, we have the following result. 
%As an example consider the function $f(x,y)=(x+y)^2$ where $\mathcal{N}(f)=\{(x,-x)|x\in\mathbb R\}$. 
%\footnote{This condition on the NE set of the objective function holds for many practical problems.}

\begin{theorem}\label{isolated_point}\textcolor{red}{maybe delete this}
Under the assumptions of \cref{bounded_to_converge}, if $\mathcal{N}(f)$ is the union of isolated points, i.e., there exists $\eta>0$, such that $\min_{\substack{y\neq z\in\mathcal{N}(f)}}\|y-z\|\geq\eta$, then $\{x^t\}$ converges to a point in $\mathcal{N}(f)$.
\end{theorem}

%\begin{remark}
%    The above convergence results are based on an assumption that the iterates are bounded. This might not hold in general. For instance, consider \begin{small}$f(x,y)=(x+y)^2+\frac{1}{2}\exp{(-(x-y)^2)}$\end{small}. This function is $2$-sided PL but the iterates of the BCD algorithm for this function are unbounded almost surely when the initial point is chosen randomly.  Note that the NE set of this function contains (0,0) and two unbounded points $\{(-\infty,\infty),(\infty,-\infty)\}$. 
%\end{remark}


It is noteworthy that, following the results of \citet{lee2016gradient,lee2019first,panageas2016gradient,ahn2022understanding}, when the function is smooth, and the initial points are chosen randomly, the BCD algorithm avoids strict saddle points in the NE set almost surely. See the Appendix \ref{sec:almostsurely} for formal statements and proofs. 

Although the above results ensure the convergence of BCD when the function is lower bounded and also satisfies the $n$-sided PL, they do not specify the last-iterate convergence rate. Unlike the two-sided PL condition that leads to linear convergence of AGDA to the min-max, the $n$-sided PL condition does not necessarily lead to any specific convergence rate of the BCD. 
To demonstrate this phenomena, we consider two $2$-sided PL functions: $f_1(x,y)=(x+y)^2+\exp(-1/(x-y)^2)$ for $(x,y)\neq (0,0)$ and zero otherwise and $f_2(x,y)=(x+y)^2$. 
% $f_1(x,y)=\left\{\begin{aligned}
    % &(x+y)^2+e^{-\frac{1}{(x-y)^2}},& \mathrm{if} (x,y)\neq (0,0)\\
    % &0,& \mathrm{if} (x,y)=(0,0)
% \end{aligned} \right.$, 
%This function is continuous and has a global minimum at $(x,y)=(0,0)$. 
We applied the BCD algorithm to both these functions with small enough\footnote{Different learning rates were selected, all less than $1/L_c$, where \( L_c \) is defined in \cref{derivative_Lip}.} constant learning rates to find their NE points with different random initializations. 
\begin{figure}
    \centering
    \includegraphics[width=6cm,height=3.3cm]{bcd_low.png}
    \caption{The BCD algorithm applied to functions $f_1(x,y)$ and $f_2(x,y)$. The y-axis is in log scale, thus the BCD demonstrates linear convergence for $f_2$.}\label{bcd_low}
    \vspace{-.3cm}
\end{figure} 
As it is illustrated in Figure \ref{bcd_low}, the BCD converges linearly for the function $f_2$ while it converges sub-linearly for $f_1$.
%randomly initiate the iterates and run the BCD 10 times. For \cref{bcd_low}, it converges slowly as the number of epochs increases compared to $f_2(x,y)=(x+y)^2$.
This example shows that characterizing the convergence rate of the BCD\footnote{Similar behavior was also observed from the GD algorithms.
%for these two functions.
} algorithm under the $n$-sided PL condition and the smoothness might not be feasible and further assumptions on the function class are required. 
 In what follows, we study one such assumption that holds for a large class of non-convex functions and characterize the convergence rate of random BCD and GD under this additional assumption.


\subsection{ Convergence under an additional assumption} 
To introduce our additional assumption, we need to define the average of the best responses
%a quantity related to function $f(x)$ 
denoted by $G_f(x)$ which plays a central role in analyzing the convergence of coordinate-wise algorithms. 
%That is the average of the best responses,
\begin{align}\label{eq:g_function}
\vspace{-.2cm}
    G_f(x):=\frac{1}{n}\sum_{i=1}^n f(x^*_i(x),x_{-i}),
    \vspace{-.2cm}
\end{align}
where $x^*_i(x)$ denotes the best response to $x_{-i}$ that is the closest to $x_i$, i.e., $x^*_i(x)\in\arg\min_{y_i}\{\|y_i-x_i\|:\ (y_i,x_{-i})\leq f(z_i,x_{-i}),\forall z_i\}$. 
It is straightforward to see that $f(x)-G_f(x)\geq 0$ for all $x$.
 Moreover, if $x^*\in\mathcal{N}_f$, the $f(x^*)=G_f(x^*)$. Conversely, if $f(x^*)-G_f(x^*)=0$, then $f(x^\star)=\min_{x_i}f(x_i,x_{-i}^\star)$, $\forall i$, which implies $x^\star\in\mathcal{N}_f$.
 
\begin{theorem}
    $x^\star$ is a NE if and only if $f(x^\star)-G_f(x^\star)=0$.
\end{theorem}
The next result shows that $G_f(x)$ is both differentiable and smooth under the $n$-sided PL condition. %See \cref{proof:G_smooth} for a proof. 
\begin{lemma}\label{G_smooth}
    If $f(x)$ satisfies $n$-sided $\mu$-PL and satisfies \cref{L_Lip}, then $\nabla G_f(x)$ exists and it is $L'$-Lipschitz, where $L':=L+\frac{L^2}{\mu}$.
\end{lemma}
Note that if function $f(x)$ is $L$-smooth and $n$-sided $\mu$-PL, then $L\geq \mu$ (see Appendix \ref{sec:tech}).  
Below, we introduce an additional assumption on $f$ under which the random BCD algorithm achieves a linear convergence rate. This is about how the gradients of $f$ and $G_f$ are aligned  
\begin{assumption}\label{ass:new}\textcolor{red}{maybe delete this}
For a given set of points $\{x^1,x^2,...\}$, there exists $0\leq\kappa<1$ such that for all $\tau$,
\begin{align}\label{eq:additional_as}
    \langle\nabla G_f(x^\tau),\nabla f(x^\tau)\rangle\leq\kappa \|\nabla f(x^\tau)\|^2.
\end{align}
\end{assumption}
For example, $f_0$ depicted in Figure \ref{fig:example1} satisfies this assumption for all points within $\{(x,y)\!:\! |x|\!>\!0.75, |y|\!>\!0.75\}$. Note that this set contains both local minimums of $f_0$.

\begin{theorem}\label{convergence_ideal_kt0}
Suppose $f(x)$ is $n$-sided $\mu$-PL satisfying \cref{L_Lip} and \cref{ass:new} \color{red}{$\langle\nabla G_f(x^\tau),\nabla f(x^\tau)\rangle\leq\kappa \|\nabla f(x^\tau)\|^2$, where $\kappa<1$ for all the iterates}, then random BCD with $\alpha^t:=\alpha\leq\frac{2(1-\kappa)}{2L'+(1+\kappa)L}$ achieves linear convergence rate, i.e., 
\begin{small}
\begin{equation*}
    \mathbb{E}[f(x^{t+1})-G_f(x^{t+1})] \leq \Big(1-\frac{\mu\alpha(1-\kappa)}{2}\Big)\mathbb{E}[f(x^t)-G_f(x^t)].
\end{equation*}
\end{small}
The expectation is taken over the randomness inherent in the procedure for selecting coordinates.
\end{theorem}
\textcolor{red}{delete this GD discussion} Similar convergence rate can be achieved using GD algorithm, i.e., $x^t=x^{t-1}-\alpha^t\nabla f(x^{t-1})$. See Appendix \ref{app:gd}.  
Under the \cref{ass:new}, the linear convergence of  $\mathbb{E}[f-G_f]$ is guaranteed using random BCD.
%the stochastic gradient descent on the $\nabla_{i^t} f(x^t)$. 
This assumption is correlated with the local strong convexity. 
Next, we show that around every isolated minimum of strongly convex and smooth functions, Assumption \ref{ass:new} holds on average for all iterates of the GD algorithm.

\begin{theorem}\label{thm:avergae_case3}
If $x^\star$ is the isolated local minimum in $U$ and $G_f$ exists, then there exists a radius $r>0$ s.t. $\forall x_0\in\mathcal{B}(x^\star,r)\subseteq U$ and by following the dynamics $\dot{r}(t)=-\nabla f(x)|_{x=r(t)}$, $r(0)=x_0\in U$, we have
\begin{equation*}
  \int_0^{+\infty}\!\!\!\! \langle\nabla G_f(x), \nabla f(x)\rangle\big|_{x=r(t)} dt \leq\! \! \int_0^{+\infty}\!\!\!\!\!\! \|\nabla f(x)\|^2\big|_{x=r(t)} dt.
\end{equation*}
Furthermore, if $\nabla^2 f(x^\star)$ is positive definite, $\nabla^2 f$ is continuous, and $f$ is $L$-smooth, then there is $0\leq \kappa<1$, s.t.
\begin{equation*}
        \int_0^{+\infty}\!\!\!\!\langle\nabla G_f(x), \nabla f(x)\rangle\big|_{x=r(t)} dt
        \leq\!\kappa\!\!\int_0^{+\infty}\!\!\!\!\|\nabla f(x)\|^2\big|_{x=r(t)}dt.
\end{equation*}    
% \begin{equation*}
% \begin{aligned}
%         &\int_0^{+\infty}\langle G_f(x), \nabla f(x)\rangle\big|_{x=r(t)} dt\\
%         \leq&\int_0^{+\infty}\left(1-\frac{\lambda_{min}^2(\nabla^2 f(x^\star))}{2nL^2}\right)\|\nabla f(x)\|^2\big|_{x=r(t)}dt.
% \end{aligned}
% \end{equation*}    
\vspace{-.3cm}
\end{theorem}



Applying the Cauchy-Schwarz inequality leads to a stronger assumption than \cref{ass:new} that is there exists $0\leq\kappa<1$, such that
%, it is straightforward to see that a stronger assumption than \cref{ass:new} is that there exists $0\leq\kappa<1$, such that
$\|\nabla G_f(x^t)\|\leq\kappa \|\nabla f(x^t)\|$. 
On the other hand, the following result shows that $\|\nabla G_f\|$ is always bounded from above by $\|\nabla f\|$ for $n$-sided PL function $f$, but with a constant greater than one. 
The constant being greater than one in this result is a consequence of the proof's construction.
%This means that very likely 
Thus, for instance, if the function $f$ is such that this constant is less than one for the iterates of the random BCD, then linear convergence can be guaranteed by \cref{convergence_ideal_kt0}. This is indeed the case for functions such as $f_0$ and the linear residual network problem (see Section \ref{sec:applications}). 
%Moreover, as we showed in Appendix \ref{sec:dis_assump}, there exists a neighborhood around every isolated local minimum of smooth functions such that, on average, the condition in \eqref{eq:additional_as} holds for all iterates of the GD dynamics.
\begin{lemma}\label{G_deri_bound}
   \textcolor{red}{maybe delete this}For an $n$-sided $\mu$-PL function $f(x)$ satisfying \cref{L_Lip}, let $C_{f}:=\frac{L}{\sqrt{n}\mu}+1$, then $\|\nabla G_f(x)\|\leq C_{f}\|\nabla f(x)\|$, for all $x$.
\end{lemma}


\subsection{Convergence with the exact best responses but without additional assumption}
Herein, we study the setting in which \cref{ass:new} does not hold. As we discussed earlier, in this setting, the BCD and GD algorithms may demonstrate different convergence rates. 
Thus, our objective in the remainder of this section is to develop variants of the random BCD and GD algorithms so that close to linear convergence is still achievable. 
To do so, we design algorithms equipped with the knowledge of the best responses, $\{x^*_i(x^t)\}$, at each iteration $t$.
More precisely, we initially propose an algorithm that presume access to the exact values of the best responses at each iteration. 
Subsequently, we refine this assumption by integrating a sub-routine into the proposed algorithm capable of approximating the best responses.
For the sake of simplicity and space, we describe our block coordinate variants here and the GD variants and their convergence analysis are presented in the Appendix \ref{sec:adaptive_alg}. 
To present our theoretical result, we need the following definition.
\begin{definition} [$(\theta,\nu)$-PŁ condition]
 The function $f$ with $\min_x f(x)=0$ satisfies $(\theta,\nu)$-PL condition iff there exists $\theta \in[1,2)$ and $\nu>0$ such that $\|\nabla f(x)\|^\theta \geq(2 \nu)^{\theta / 2} f(x). \quad$    
\end{definition}
It has been proved by \citet{lojasiewicz1963topological} that for any $C^1$ analytic function, there exists a neighborhood $U$ around the minimizer where $(\theta,\nu)$-PL condition is satisfied.

\begin{algorithm}[tb]
   \caption{Ideal Adaptive Randomized Block Coordinate Descent (IA-RBCD)}
\begin{algorithmic}\label{arbcd_ideal}
   \STATE {\bfseries Input:} initial point $x^0=(x_1^0,...,x_n^0)$, $T$, learning rates $\alpha$, $0\leq\gamma<1$ and $C>0$
   \FOR{$t=0$ {\bfseries to} $T-1$}
   \STATE sample $i^t$ uniformly from $\{1,2,...,n\}$
   %\STATE compute $\nabla G(x^t)=\frac{1}{n}\sum_{l=1}^n\nabla \min_{x_i}f(x_i,x_{-i}^{t})$
   \IF{$\langle\nabla G_f(x^t),\nabla f(x^t)\rangle \leq \gamma \|\nabla f(x^t)\|^2$}
   \STATE $k^t=0$ \hfill\texttt{:Case 1:}
   \ELSIF{$\frac{(\|\nabla G_f(x^t)\|^2-\langle\nabla f(x^t),\nabla G(x^t)\rangle)^2}{\langle\nabla f(x^t),\nabla G(x^t)\rangle^2}>C$}
   \STATE $k^t=-2+\frac{\langle\nabla f(x^t),\nabla G_f(x^t)\rangle}{\|\nabla G_f(x^t)\|^2}$ \hfill\texttt{:Case 2:}
   \ELSE   \STATE $k^t=-1$ \hfill\texttt{:Case 3:}
   \ENDIF
   \STATE $x_{i^t}^{t+1}=x_{i^t}^{t}-\alpha(\nabla_{{i^t}}f(x^{t})+k^t\nabla_{i^t}G_f(x^t)), \quad x_{i}^{t+1}=x_{i}^{t}$ if $i\neq i^t$
   \ENDFOR
   %\STATE {\bfseries Output:} $x^{T}=(x_1^{T},...,x_n^{T})$
\end{algorithmic}
\end{algorithm}
Algorithm \ref{arbcd_ideal} presents the steps of our modified version of the random BCD. In this algorithm, instead of updating along the direction of $-\nabla_{i^t} f(x)$, where $i^t$ denotes the chosen coordinate at iteration $t$, a linear combination of $\nabla_{{i^t}}f(x)$ and $\nabla_{i^t}G_f(x)$ is used to refine the updating directions.
The coefficient of this linear combination, \(k^t\), is adaptively selected based on the current estimated point. 
It is important to mention that $\nabla G_f(x)$ can be computed using the gradient of $f$ and the best responses, i.e., 
\begin{small}
\vspace{-.3cm}
\begin{align}\label{eq:gradient_g}
    \nabla G_f(x)=\frac{1}{n}\sum_{i=1}^n\nabla f\big(x^*_i(x), x_{-i}\big).
\end{align}
\end{small}


\begin{theorem}\label{convergence_ideal}
\vspace{-.2cm}
For $n$-sided $\mu$-PL function $f(x)$ satisfying \cref{L_Lip}, by applying \cref{arbcd_ideal}, 
\begin{itemize}[leftmargin=8pt]
    \item in Case 1 with $\alpha\!\leq\!\frac{2(1-\gamma)}{2L'+(1+\gamma)L}$, we have 
\footnotesize{$\mathbb{E}[f(x^{t+1})\!-\!G_f(x^{t+1})|x^t]\! \leq\! \big(1\!-\!\frac{\mu\alpha(1-\gamma)}{2}\big)(f(x^t)\!-\!G_f(x^t)),$}

\item in Case 2 with $\alpha\!\leq\min\{\frac{1}{2(L+L')},\frac{C}{2(L+L')}\}$, we have
\footnotesize{$\mathbb{E}[f(x^{t+1})\!-\!G_f(x^{t+1})|x^t]\!\leq\!\! \Big(1\!-\!\!\frac{(L+L')\mu\alpha^2}{2}\Big)(f(x^t)\!-\!G_f(x^t)),$}

\item in Case 3 with $\alpha\!\leq\!\frac{1}{L+L'}$, $f-G_f$ is non-increasing. Furthermore, if $f-G_f$ satisfies $(\theta,\nu)$-PL condition and case 3 are satisfied from iterates $t$ to $t+k$, we have
\begin{small}
\begin{equation*}
    \mathbb{E}[f(x^{t+k})-G_f(x^{t+k})|x^t]\leq\mathcal{O}\Big(\frac{f(x^{t})-G_f(x^{t})}{k^{\frac{\theta}{2-\theta}}}\Big).    
\end{equation*}
\end{small}
\end{itemize}
\vspace{-.4cm}
\end{theorem}
The exact constant terms are provided in the proof. 
According to this result, IA-RBCD in \ref{arbcd_ideal} demonstrates linear rate for two out of three cases and sub-linear rate for the third case. Next, we show that even if the third case occurs frequently
%When the third case occurs finitely many times, e.g., for a neighborhood around an isolated NE point, the third case does not occur 
(e.g., function $f_0$ in Figure \ref{fig:example1}), then linear converge is guaranteed by IA-RBCD. 
Next, we analyze the rarity of case 3 and in Section \ref{sec:applications}, empirically verify this rarity for several well-known problems.
%Since rigorously verifying these cases is intractable, we empirically verify them for different well-known problems in the next section.

% \textcolor{blue}{
% Prove a corollary or a proposition that shows even if we visit case 3, $\alpha T$ rounds for any $\alpha<1$, the convergence rate still would be linear. 
% }

\begin{theorem}\label{case_many_enough}
    Under the assumptions of \cref{convergence_ideal}, by applying Algorithm \ref{arbcd_ideal} for $t$ iterations and denoting the number of iterations, it visits Case 3 by $b(t)$($\leq t$), if
    $ B:=\lim\sup_{t\to +\infty} b(t)/t<1$,
    then $\forall\epsilon$ such that $0<\epsilon< 1-B$, there exists $\hat{t}$ such that for all $t\geq \hat{t}$,
    \begin{equation*}
        \mathbb{E}[f(x^t)-G_f(x^t)]\leq c^{t}\cdot(f(x^0)-G_f(x^0)),
    \end{equation*}
     where $c\!:=\!\big(\min\{1-\frac{\mu\alpha(1-\kappa)}{2},1-\frac{(L+L')\mu\alpha^2}{2}\}\big)^{1-B-\epsilon}\!\!<1$.
\end{theorem}

In the following theorem, we demonstrate as $\gamma \to 1$ and $C \to 0$, the measure of non-NE points that fail to satisfy case 1 and case 2 converges to zero and when the iterates fall into case 3, $f-G_f$ is small at those iterates.

\begin{theorem}\label{thm:measure}
    If $f(x)$ satisfies the assumption of \cref{convergence_ideal}, then, by defining $S(\gamma, C)$ to be the set of non-NE points that do not satisfy case 1 and case 2, we have
    \begin{equation*}
        \lim_{\gamma\to 1, C\to 0} |S(\gamma,C)|=0,
        \vspace{-.1cm}
    \end{equation*}
    where $|S(\gamma, C)|$ denotes the measure of the set $S(\gamma, C)$. Moreover, if $S(\gamma,C)$ is non-empty, then
        $\lim_{\gamma\to 1, C\to 0} \max_{x\in S(\gamma, C)}f(x)-G_f(x)=0$.
\end{theorem}

It is crucial to highlight that BCD requires \cref{lower-bounded} to converge to the NE \citep{xu2013block} and almost surely avoids strict saddle points \citep{lee2016gradient}. However, \cref{convergence_ideal} shows that IA-RBCD converges to the NE, irrespective of these conditions.

\vspace{-.1cm}
\subsection{Convergence with approximated best responses and without additional assumption}
Evaluating $G_f$ at a given point requires the knowledge of the best responses at that point. Often, these best responses are not known a priori and they have to be computed at each iteration.  
Fortunately, since in our study, $f$ satisfies the $n$-sided PL condition, the best responses can be efficiently approximated, by applying GD algorithm with the partial gradients as a sub-routine.
Algorithm \ref{sub-routine} in the Appendix presents the steps of this sub-routine and Algorithm \ref{arbcd_practical} shows the steps of our adaptive random BCD algorithm. 
The main difference between algorithms \ref{arbcd_ideal} and \ref{arbcd_practical} is that at every iteration, A-RBCD approximates the best responses function by gradient descent. 
%This is efficient as it converges to the $G_f$ at a linear rate. 
According to the next result, the number of steps for approximating $G_f$, $T'$, only depends on the function parameters and it is independent of the final precision of $f-G_f$. 
%In other words, to achieve $f(x)-G_f(x)\leq \epsilon$, we only need $O(\log(1/\epsilon))$ steps of computing gradient.
\begin{theorem}\label{convergence_practical}
For an $n$-sided $\mu$-PL function $f(x)$ satisfying \cref{L_Lip}, by implementing \cref{arbcd_practical} with $\beta\leq\frac{1}{L}$ and $T'\geq\log\big(\frac{169nL^2}{\mu^2\gamma^2\alpha^6}\big)/\log(\frac{1}{1-\mu\beta})$, 
\vspace{-.2cm}
\begin{itemize}[leftmargin=7pt]
\item in Case 1 with $\alpha\!\leq\!\frac{2(1-\gamma)}{2L'+(1+\gamma)L}$, we have
\begin{small}
$
\mathbb{E}[f(x^{t+1})-G_f(x^{t+1})|x^t]\leq (1-\frac{\mu\alpha(1-\gamma)}{2})(f(x^t)-G_f(x^t)),
$
\end{small}

\item in Case 2 with \begin{small}$\alpha\leq\min\big\{(\frac{3C\gamma}{(13+12\gamma)C_{f}})^{1/2}$, $\frac{1}{C_{f}^{1/2}},\frac{71C\gamma^2}{676(L+L')}, \frac{3\gamma(L+L')\mu}{(13+108\gamma)LC_{f}^4},$ $\frac{1}{2(L+L')}\big\}$\end{small}, we have
\begin{small}
\begin{equation*}
    \mathbb{E}[f(x^{t+1})-G_f(x^{t+1})|x^t]\leq C_0\cdot(f(x^t)-G_f(x^t)),
\end{equation*}
\end{small}
where $C_0:=(1-\frac{(L+L')\mu\alpha^2}{4})$.

\item in Case 3 with  $f\!-\!G_f$ is non-increasing when $\alpha\!\leq\!\min\!\big\{\frac{1}{L+L'}$, $(\frac{13}{12(1+C_{f})})^{1/3}\frac{\|\nabla f(x^t)-\nabla G_f(x^t)\|}{\|\nabla f(x^t)\|}\big\}$. Furthermore, if $f\!-\!G_f$ satisfies $(\theta,\nu)$-PL condition and case 3 occurs from iterates $t$ to $t+k$, then
\begin{small}
\begin{equation*}
    \mathbb{E}[f(x^{t+k})-G_f(x^{t+k})|x^t]\leq\mathcal{O}\Big(\frac{f(x^{t})-G_f(x^{t})}{k^{\frac{\theta}{2-\theta}}}\Big)
\end{equation*}
\end{small}

\end{itemize}
\end{theorem}
\begin{algorithm}[tb]
   \caption{Adaptive randomized Block Coordinate Descent (A-RBCD)}
\begin{algorithmic}\label{arbcd_practical}
   \STATE {\bfseries Input:} initial point $x^0=(x_1^0,...,x_n^0)$, $T, T'$,  learning rates $\alpha$, $\beta$, $0<\gamma<1$ and $C>0$
   \FOR{$t=0$ {\bfseries to} $T-1$}
   \STATE sample $i^t$ uniformly from $\{1,2,...,n\}$
   \STATE $y^{t,T'}=$ABR$(x^{t}, T', \beta)$ \hfill \texttt{:Algorithm \ref{sub-routine}}
   \STATE compute $\tilde\nabla G_f(x^t)=\frac{1}{n}\sum_{l=1}^n\nabla f(y_l^{t,T'},x_{-l}^{t})$
   \IF{$\langle\tilde\nabla G_f(x^t),\nabla f(x^t)\rangle\leq (\gamma-\gamma\frac{\alpha_t^{3}}{13}) \|\nabla f(x^t)\|^2$}
   \STATE $\tilde k^t=0$ \hfill\texttt{:Case 1:}
   \ELSIF{$\frac{(\|\tilde\nabla G_f(x^t)\|^2-\langle\nabla f(x^t),\tilde\nabla G_f(x^t)\rangle)^2}{\|\tilde\nabla G_f(x^t)\|^4}>C$ }
   \STATE $\tilde k^t=-2+\frac{\langle\nabla f(x^t),\tilde\nabla G_f(x^t)\rangle}{\|\tilde\nabla G_f(x^t)\|^2}$\hfill\texttt{:Case 2:}
   \ELSE
   \STATE $\tilde k^t=-1$ \hfill\texttt{:Case 3:}
   \ENDIF
   \STATE $x_{i^t}^{t+1}=x_{i^t}^{t}-\alpha(\nabla_{i^t}f(x^{t})+\tilde k^t\tilde\nabla_{i^t}G_f(x^t)), \quad x_{i}^{t+1}=x_{i}^{t}$, if $i\neq i^t$
   \ENDFOR
   %\STATE {\bfseries Output:} $x^{T}=(x_1^{T},...,x_n^{T})$
\end{algorithmic}
\end{algorithm}



%\begin{algorithm}[tb]
%   \caption{Adaptive randomized Block Coordinate Descent (A-RBCD)}
%\begin{algorithmic}\label{arbcd_practical}
%   \STATE {\bfseries Input:} initial point $x^0=(x_1^0,...,x_n^0)$, positive number $\{\alpha_t\}$, $\beta$, $C$ and $\gamma<1$
%   \FOR{$t=0$ {\bfseries to} $T-1$}
%   \STATE sample $i^t$ uniformly from $\{1,2,...,n\}$
%   \FOR{$j=1,...,n$}
%   \STATE $y_j^{t,0}=x_{j}^{t}$
%   \FOR{$t_i=0,...,T'-1$}
%   \STATE $y_j^{t,t_i+1}=y_j^{t,t_i}-\beta\nabla_{j}f(y_j^{t,t_i},x_{-j}^{t})$
%   \ENDFOR
%   \ENDFOR
%   \STATE compute $\tilde\nabla G_f(x^t):=\frac{1}{n}\sum_{l=1}^n\nabla f(y_l^{t,T'},x_{-l}^{t})$
%   \IF{$\langle\tilde\nabla G_f(x^t),\nabla f(x^t)\rangle\leq (\gamma-\gamma\frac{\alpha_t^{3}}{13}) \|\nabla f(x^t)\|^2$}
%   \STATE $\tilde k^t=0$ \hfill\texttt{:Case 1:}
%   \ELSIF{$\frac{(\|\tilde\nabla G_f(x^t)\|^2-\langle\nabla f(x^t),\tilde\nabla G_f(x^t)\rangle)^2}{\|\tilde\nabla G_f(x^t)\|^4}>C$ and $\langle\tilde\nabla G_f(x^t),\nabla f(x^t)\rangle\geq (\gamma-\gamma\frac{\alpha_t^{3}}{13}) \|\nabla f(x^t)\|^2$ {\color{blue} This should hold as it is in the elseif!?}}
%   \STATE $\tilde k^t=-1+\frac{\langle\nabla f(x^t),\tilde\nabla G_f(x^t)\rangle-\|\tilde\nabla G(x^t)\|^2}{\|\tilde\nabla G_f(x^t)\|^2}$\hfill\texttt{:Case 2:}
%   \ELSE
%   \STATE $\tilde k^t=-1$ \hfill\texttt{:Case 3:}
%   \ENDIF
%   \STATE $x_{i^t}^{t+1}=x_{i^t}^{t}-\alpha_t(\nabla_{i^t}f(x^{t})+\tilde k^t\tilde\nabla_{i^t}G_f(x^t)), \quad x_{i}^{t+1}=x_{i}^{t}$, if $i\neq i^t$
%   \ENDFOR
%   \STATE {\bfseries Output:} $x^{T}=(x_1^{T},...,x_n^{T})$
%\end{algorithmic}
%\end{algorithm}






==> Applications.tex <==
\vspace{-.5cm}
\section{Applications}\label{sec:applications}
Herein, we discuss two well-known nonconvex problems that satisfy the $n$-sided PL condition.

\textbf{Function with only strict saddle point: } We consider the function $f(x,y)=(x-1)^2+4(x+0.1\cos(x))y+(y+0.1\sin(y))^2$. The problem aims at finding the NE $(x^\star,y^\star)$, 
\begin{equation*}
\begin{aligned}
    f(x^\star,y^\star)\leq f(x,y^\star),\forall x,\quad     f(x^\star,y^\star)\leq f(x^\star,y),\forall y.    
\end{aligned}
\vspace{-.3cm}
\end{equation*}

\begin{figure}
\centering
\subfigure[]{
\includegraphics[width=0.45\linewidth,height=2.8cm]{non_convergence.png}}
\subfigure[]{
\includegraphics[width=0.45\linewidth,height=2.6cm]{strict_saddle.png}}
\caption{(a) Performance of A-RBCD (blue) and BCD (red) on function $f(x,y)$ shown in (b).}\label{fig:non_convergence}
\vspace{-.3cm}
\end{figure}
Figure \ref{fig:non_convergence} represents the convergence results of A-RBCD and BCD with 100 random initialization. 
The iterates of A-RBCD always converge to the NE at a linear rate, while BCD diverges. Note that the NE is a strict saddle point.  

\textbf{Linear Residual Network: } It aims to learn the linear transformation $R:\mathbb{R}^d \rightarrow\mathbb{R}^d$, such that $y=Rx+\xi$, where $\xi\sim \mathcal{N}(0,I_d)$ and $I_d$ denotes the identity matrix of dimension $d$. The learned model can be parameterized by a sequence of weight matrices $A_1,..., A_n\in\mathbb{R}^{d\times d}$, such that
$h_0=x$, $h_j=(I+A_j)h_{j-1}$, $\hat{y}=h_n$. 
Thus, the objective function of this problem is given by
\begin{equation*}
\begin{aligned}
        f(A_1,...,A_n):&=\mathbb{E}[\|\hat{y}-y\|^2]\\
        &=\mathbb{E}\big[\|(I+A_n)...(I+A_1)x-Rx-\xi\|^2\big].
\end{aligned}
\end{equation*}
Even though $(I+A_n)\cdots(I+A_1)$ is a linear map, the optimization problem onhe factored variables $(A_1,..., A_n)$ is nonconvex \citep{hardt2016identity}. %{As we have shown in \cref{proof:LRN_convergence}, this function satisfies both the $n$-sided PL condition if $\max_i\|A_i\|<1$, and Assumption \ref{ass:new}. Thus, linear convergence can be achieved using both random BCD and A-RBCD. We also demonstrated this through empirical evidence.}
More precisely, we considered two settings: (1) $d=3, n=5$ and (2) $d=5, n=10$ with covariance matrices $\Sigma=\mathbb{E}[xx^T]=I_d$, and applied the A-RBCD algorithm to both settings. 
Figure \ref{fig:exp1} illustrates the resulting error curves on a log-scaled y-axis, obtained from 100 trials. Each trial is obtained by randomly selecting the diagonals of matrix $R$ according to $U(0.5,1.5)$ and initializing $A_i$s with random entries according to $U(-0.1,0.1)$. 
\begin{figure}
\centering  
\subfigure[$n=5, d=3$]{
\includegraphics[width=0.47\linewidth,height=2.8cm]{5_LRN.png}}
\subfigure[$n=10, d=5$]{
\includegraphics[width=0.47\linewidth,height=2.8cm]{10_LRN.png}}
\caption{Performance of the A-RBCD and RBCD on linear residual network problems for different network sizes illustrates linear convergence, as advocated by \cref{convergence_ideal_kt0}.}\label{fig:exp1}
\vspace{-.3cm}
\end{figure}

\vspace{-.1cm}
\textbf{Infinite Horizon $n$-player Linear-quadratic (LQR) Game:} 
The objective function is formulated as 
\begin{small}
\begin{equation*}
    \mathbb{E}_{x_0\sim\mathcal{D}}\big[\sum_{t=0}^{+\infty}[(x^t)^T Q x^t+\sum_{i=1}^n ((u_i^t)^T R_i u_i^t]\big],
\end{equation*}
\end{small}
where $x_t$ denotes the state, $u_i^t$ is the input of $i$-th player at time $t$, and $i\in[n]$. The state transition of the system is characterized by 
$x^{t+1}=Ax^t+\sum_{i=1}^n B_iu_i^t$, where $A\in\mathbb R^{k\times k}$ and $B\in\mathbb R^{k\times d}$.
When players apply linear feedback strategy, i.e., $u_i^t=-K_i x^t,$, the objective function becomes 
\begin{small}
\begin{equation*}
    f(K_i,K_{-i})=\mathbb{E}_{x_0\sim\mathcal{D}}\big[\sum_{t=0}^{+\infty}[(x^t)^T Q x^t+\sum_{i=1}^n ((K_ix_i^t)^T R_i K_ix_i^t]\big].
\end{equation*}
\end{small}
If $K_i$s are bounded and $\Sigma_0=\mathbb{E}_{x^0\sim\mathcal{D}}[x^0(x^0)^T]$ is full rank, the objective function $f$ satisfies the $n$-sided PL condition (see  \cref{proof_n_sided_LQR} for a proof). 
However, as it is discussed in \cite{fazel2018global}, even the objective of one-player LQR is not convex. Subsequently, the objective function of the $n$-player LQR game is not multi-convex. See \cref{ce_LQR_convex} for examples.

\begin{figure}
\subfigure[\footnotesize{$n=5$,\ $d=3$}]{
\includegraphics[width=0.45\linewidth]{5.png}}
\subfigure[\footnotesize{$n=10$,\ $d=5$}]{
\includegraphics[width=0.45\linewidth]{10.png}}
\\
\subfigure[\footnotesize{$n=20$,\ $d=10$}]{
\includegraphics[width=0.45\linewidth]{20.png}}
\subfigure[\footnotesize{$\rho$}]{
\includegraphics[width=0.45\linewidth]{rho.png}}
\caption{Performance of the A-RBCD and RBCD on  LQR for different game sizes. The y-axis of (a)-(c) are in the log scale.}\label{fig:lqr}
\vspace{-.3cm}
\end{figure}
We applied our A-RBCD algorithm to this problem when $A\in\mathbb{R}$,  $B_i\in\mathbb{R}^{1\times d}$ and the entries of $B_i$, $Q$ and the diagonal entries of $R_i$ were sampled according to $\frac{1}{nd}U(0,1)$, $U(0,1)$ and $U(0,1)$, respectively. 
%{\color{blue}
%$\frac{1}{30}\mathcal{N}(0,1)$ has a variance of 1/900 which is very small, That means most of the entries of B are zeros. is that correct?}
%where $\mathcal{N}(0,1)$ represents the normal distribution with mean 0 and variance 1, and $U(0,1)$ represents the uniform distribution between 0 and 1. 
We set the learning rate $\alpha$= 0.05 and random initialization $K_i\!\sim\! U(0,1)^d$ for all $i$. 
Fig. \ref{fig:lqr} demonstrates the resulting error curve, $f(K^t)\!-\!G_f(K^t)$, 
%, the norm of their difference $\|K^t-K^\star\|_F$, 
and $\rho\!:=\!\frac{\langle\nabla f(K^t),\nabla G_f(K^t)\rangle}{\|\nabla f(K^t)\|^2}$. This shows that during the updating procedure, the third case did not occur. 
Plots are obtained from 50 trials. 


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{nips/ratio_2.eps}
%     \caption{The ratio $\frac{\langle\nabla f(K^t),\nabla G_f(K^t)\rangle}{\|\nabla f(K^t)\|^2}$}
% \end{figure}

==> Assumptions.tex <==
\vspace{-.1cm}
\subsection{Definitions and Assumptions}\label{sec:def}

%In this section, we introduce a set of necessary assumptions under which we can guarantee the convergence of our algorithm. 

Throughout this paper, we assume the function $f(x):$ $\mathbb{R}^d\to\mathbb{R}$ belongs to $C^1$, i.e., it is continuously differentiable. Furthermore, we assume it has a Lipschitz gradient.% We state it as a basic assumption.

\begin{assumption}[Smoothness]\label{L_Lip}
We assume the $L$-Lipschitz continuity of the derivative $\nabla f(x)$,
\begin{equation*}
    \|\nabla f(x)-\nabla f(y)\|\leq L\|x-y\|, \forall x, y
\end{equation*}
where $L>0$ is a constant. In this case, $f(x)$ is also called $L$-smooth.
\end{assumption}

A slightly weaker assumption is coordinate-wise smoothness given below. Note that under the Lipschitz gradient assumption, the coordinate-wise smoothness can be deduced.
\begin{assumption}[Coordinate-wise Smoothness]\color{red}{maybe delete this.}\label{derivative_Lip}
We assume the coordinate-wise $L_c$-Lipschitz continuity of the derivative $\nabla f(x)$, that is for all $x_i,x_i',x_{-i}$ and $i\in[n]$,
\begin{equation*}
\begin{aligned}
    \|\nabla_{i} f(x_i,x_{-i})-\nabla_{i} f(x_i',x_{-i})\|\leq L_c\|x_i-x_i'\|,
\end{aligned}
\end{equation*}
where $L_c>0$ is a constant. In this case, $f(x)$ is also called a coordinate-wise $L_c$-smooth function.
\end{assumption}

\begin{assumption}[Lower bounded]\label{lower-bounded}
The function $f(x)$ is lower bounded, i.e. $\inf_{x\in\mathbb{R}^{d}} f(x)>-\infty$.
\end{assumption}


We now define two notions of optimality for the minimization problem in \cref{min_problem}; Nash Equilibrium (NE) and Stationary point. 
%One of the notions of optimality is Nash Equilibrium, at which $x_i^{\star}$ is an optimal solution to the function $f_i(x)=f(x,x_{-i}^\star)$ for all $i\in[n]$.

\begin{definition}[Nash Equilibrium (NE)]
 Point $x^\star=(x_1^\star,...,x_n^\star)$ is called a Nash Equilibrium of function $f(x)$ if 
 \begin{equation*}
     f(x_{i}^\star,x_{-i}^\star)\leq f( x_{i},x_{-i}^\star), \forall i\in[n], \forall x_i\in\mathbb{R}^{d_i}.
 \end{equation*}
The set of all NE points of $f(x)$ is denoted by $\mathcal{N}(f)$.
\end{definition}
The other notion, stationary point, is related to the first-order condition of optimality and also relevant for studying gradient-based algorithms.

%\begin{definition}[Stationary Point]
%    A point $x^\star$ is a stationary point if
%    \begin{equation}
%        \nabla f(x^\star)=0.
%    \end{equation}
%\end{definition}
\begin{definition}[$\varepsilon$-Stationary point]\color{red}{why $\epsilon$ needs to be nonzero here?}
    Point $\tilde x=(\tilde x_1,...,\tilde x_n)$ is called an $\varepsilon$-stationary point of $f(x)$ if 
    $
    \|\nabla f(\tilde x)\|\leq \varepsilon.
    $
    When $\varepsilon=0$, the point $\tilde x$ is called a stationary point. We denote the set of all $\varepsilon$-stationary points and the set of all stationary points of $f(x)$ by $\mathcal{S}_\varepsilon(f)$ and $\mathcal{S}(f)$, respectively.
\end{definition}
For general nonconvex minimization problems, the above two notions are not necessarily equivalent, i.e., a stationary point may not be a NE. %Since our goal in this work is to find NE, in the remainder of the paper, we assume that the function $f(x)$ has an NE.
Nevertheless, for the remainder of this work, we assume that the objective function $f$ has at least one NE, i.e., $\mathcal{N}_f\neq \emptyset$. We also assume that $\arg\min_{x_i\in\mathbb{R}^{d_i}}f(x_i,x_{-i})$ is non-empty for any $i\in[n]$ and $x_{-i}$, i.e., there exists a best response to every $x_{-i}$. Note that this is not a limiting assumption given that the function is lower bounded. 
Below, we formally introduce the $n$-sided PL condition for the function $f(x)$.
%satisfies the $\mu$-PL condition with constant $\mu$ for all $x_{-i}$. We formally state this in the following.


\begin{definition}[$n$-sided PL Condition]\label{PL_condition}
We say $f(x)=f(x_1,...,x_n)$ satisfies $n$-sided $\mu$-PL condition if there exists a positive constant $\mu>0$ such that for all $x\in\mathbb{R}^{d}, i\in[n]$
\begin{align}\label{eq:n-sided}
\|\nabla_{i}f(x_i,x_{-i})\|^2\geq 2\mu\big(f(x_i,x_{-i})-f_{x_{-i}}^\star\big), 
\end{align}   
\vspace{-.1cm}
where $f_{x_{-i}}^\star:=\min_{y_i} f(y_i,x_{-i})$.    
\end{definition}


%We say a function $f(x)$ is $n$-sided PL, if it satisfies the $n$-sided $\mu$-PL condition for some $\mu>0$. 
It is worth noting that the $n$-sided PL condition does not imply convexity or the gradient dominance (PL) condition. It is an extension to the PL condition, as when $f$ is independent of $x_{-i}$, %i.e., $f(x_i,x_{-i})=\phi(x_i)$ for some function $\phi$ satisfying the PL condition, 
then $f$ satisfies the PL condition. Moreover, it is considerably weaker than multi-strong convexity.

Next result shows that under the $n$-sided PL condition, the set of stationary points and the NE set are equivalent. For instance, the set of stationary points and the NE set of $f_0$ in Figure \ref{fig:example1} is $\{(-1,-1), (1,1), (0,0)\}$. All proofs are in the Appendix \ref{sec:proofs}.
\begin{lemma}\label{SP_equal_NE}
If $f(x)=f(x_1,...,x_n)$ satisfies the $n$-sided PL condition, then $\mathcal{S}(f)=\mathcal{N}(f)$
\end{lemma} 
It is also important to emphasize that, unlike the $n$-sided PL, the two-sided PL condition is defined such that the right-hand side of \eqref{eq:n-sided} is the difference between the function and its minimum for one coordinate while for the other coordinate it is the difference between the function and its maximum. As a consequence, under the two-sided condition, the stationary points are also global minimax points.
However, under the $n$-sided PL condition in \cref{PL_condition}, it is no longer possible to ensure that the NE are global minimums. In fact, there could be multiple NEs with different function values. For example, consider the functions $f_0(x,y)$ and $f(x,y)$ illustrated in Figure \ref{fig:example1}. As shown in Appendix \ref{app:example}, both functions are $2$-sided PL, but their set of NE and the set of minimum points are not equivalent. 
In particular, both functions have three NE points while, $f_0(x,y)$ has two global minimums and a saddle point, and $f(x,y)$ has a local, a global minimum, and a saddle point. 
\begin{figure}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=0.44\linewidth,,height=2.1cm]{example1.jpg}
         %\caption{Function $f_0(x,y)=(x-1)^2(y+1)^2+(x+1)^2(y-1)^2$.}
         \label{fig:y equals x}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[width=0.42\linewidth,,height=2.1cm]{Example2.png}
         %\caption{Function $f(x,y)=(x-1)^2(y+1)^2+(x+1)^2(y-1)^2+\exp(-(y-1)^2)$.}
         \label{fig:three sin x}
     \end{subfigure}
        \caption{Left is function \begin{small}$f_0(x,y)\!=\!(x-1)^2(y+1)^2\!+\!(x+1)^2(y-1)^2$\end{small} and right is function \begin{small}$f(x,y)=f_0(x,y)+\exp(-(y-1)^2)$\end{small}.}
        \label{fig:example1}
\end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=5.5cm,height=3cm]{example1.jpg}
%     \caption{Function $f(x,y)=(x-1)^2(y+1)^2+(x+1)^2(y-1)^2$.}
%     \label{fig:example1}
% \end{figure}
\begin{remark}\textcolor{red}{why we need to discuss this?}
    The $n$-sided PL condition is defined coordinated-wise, with the coordinates aligned with the vectors $\{e_1,...,e_n\}$, where $e_i$ belongs to $\mathbb R^d$, such that the entries corresponding to the $i$-th block are one and zero elsewhere. 
    This condition can naturally be extended to $n$-sided directional PL in which the $i$-th inequality is aligned with a designated vector $v_i$. In this extension, the partial gradient and $f^*_{x_{-i}}$ are replaced with their directional variants along vector $v_i$. 
    Note that the results of this work will remain valid in the directional setting, provided that the definitions of NE and the presented algorithms are adjusted to their respective directional variants. 
\end{remark}
%In what follows, we study several gradient-based algorithms such as BCD and their convergences under the proposed $n$-sided $\mu$-PL condition. 




%In \cref{SP_equal_NE}, we show that the notions of stationary point is equivalent with the notion of Nash Equilibrium under the $n$-sided $\mu$-PL condition. Note that they may not be unique. 

%\begin{lemma}\label{SP_equal_NE}
%If $f(x)$ satisfies \cref{PL_condition} for some $\mu>0$, then $\mathcal{S}(f)=\mathcal{N}(f)$.
%\begin{equation}
 %   \mathrm{Stationary}\ \mathrm{Point}\Longleftrightarrow\mathrm{Nash}\ \mathrm{Equilibirum}.
%\end{equation}
%\end{lemma}














==> Conclusion.tex <==
\vspace{-.3cm}
\section{Conclusion}
\vspace{-.2cm}
In this paper, we identified a subclass of nonconvex functions called $n$-sided PL functions and studied the convergence of GD-based algorithms, particularly the BCD algorithm, for finding their NEs. The $n$-sided PL condition is a reasonable extension of the gradient dominance condition, which holds in various problems. 
We showed that the convergence rate of such first-order algorithms in this subclass of functions depends on a local relation between the function $f$ and the average of the best responses $G_f$. Subsequently, we proposed two novel algorithms, IA-RBCD and A-RBCD, equipped with $G_f$, that provably converge to the NE set almost surely with random initialization even if the function is not lower bounded and has strict saddle points. We hope this work can shed some light on the understanding of nonconvex optimization.





%In this paper, we identify a subclass of nonconvex problems with block structure, represented by the so-called $n$-sided PL condition. We also propose the first two random algorithms, IA-RBCD and A-RBCD that provably converge to the Nash Equilibrium in most of cases, while protect the privacy of every blocks. We hope this work can shed some light on the understanding of nonconvex optimization, especially the PL condition: (1) the $n$-sided PL condition is a reasonable extension for the strong PL condition, with the existence of average of best response function $G_f$; (2) the complexity of solving a nonconvex optimization problem may depends on the relation between the function $f$ and average of best response $G_f$; It remains interesting to explore whether applying similar algorithm can result in linear convergence rate to the Nash Equilibrium or even the global minimum.

==> Definitions.tex <==






==> Introduction.tex <==
\section{Introduction}

Optimization problems with nonconvex objectives appear in many applications from computer science to economics \citep{intriligator2002mathematical} and more recently, in machine learning \citep{jain2017non}, such as training deep neural networks \citep{heaton2018ian} or policy optimization in reinforcement learning \citep{silver2014deterministic}. 
On the other hand, the Gradient Descent (GD) algorithm and its variants are driving the practical success of many machine learning approaches. Naturally, understanding the limits of such GD-based algorithms in the nonconvex setting has become an important avenue of research in recent years \citep{jin2021nonconvex, zhou2018convergence,jordan2023deterministic}.
Along this line of research, we are interested in finding Nash Equilibrium $x^\star=(x_1^\star,\cdots,x_n^\star)$ of the nonconvex function $f(x)$, i.e.,
\begin{equation}\label{min_problem}
        f(x_i^\star;x_{-i}^\star)\leq f(y_i;x_{-i}^\star), \forall y_i\in\mathbb{R}^{d_i},
\end{equation}
where $f$ is a continuously differentiable but possibly nonconvex function. The variable $x$ can be partitioned into $n$ blocks $(x_1,...,x_n)$, where $x_i\in\mathbb{R}^{d_i}$ is the $i$-th block and $\sum_{i=1}^n {d_i}=d$. 
This optimization problem can be viewed as a %general-sum 
potential game between $n$ players. The objective of $i$-th player is to minimize the function $f(x_i,x_{-i})$ when other players' parameters are denoted by $x_{-i}$.


From a game-theoretic perspective, this is a multi-agent potential game where the potential function $ f $ captures the aggregate impact of  agents' strategies $ \{x_i\}_{i=1}^n $ \citep{monderer1996potential}. 
Each agent minimizes $f$ over its variables $x_i$, assuming others' strategies are fixed.
However, privacy concerns arise as strategies may reveal sensitive information. In decentralized settings, such as network routing \citet{candogan2010near} or resource allocation \citep{zhang2021potential}, agents optimize independently without full knowledge of $ f $. Furthermore, convergence to an NE is not always stable \citep{carmona2013existence}, as gradient descent may diverge.



For a general nonconvex differentiable function $f: \mathbb{R}^d\to\mathbb{R}$, finding its NE is PPAD-complete \citep{daskalakis2009complexity}. 
A straightforward approach to tackle this problem is to introduce additional structural assumptions to achieve convergence guarantees. Within this scope, various relaxations of convexity have been proposed, for example,  weak strong convexity \citep{liu2014asynchronous}, restricted secant inequality \citep{zhang2013gradient}, error bound \citep{cannelli2020asynchronous}, quadratic growth \citep{cui2017quadratic}, etc.  
Recently, there has been a surge of interest in analyzing nonconvex functions with block structure. Multiple assumptions have been analyzed which is correlated to each block when other blocks are fixed, for example, PL-strongly-concave \citep{guo2020fast}, nonconvex-PL \citep{sanjabi2018solving}, PL-PL \citep{daskalakis2020independent, yang2020global,chen2022faster} and multi-convex \citep{xu2013block,shen2017disciplined,wang2019multi,wang2022accelerated}. %However, multi-convex assumes the convexity of the function when other blocks are fixed, which is unable to deal with nonconvex scenarios. Other conditions mentioned above can only be applied when the objective function has only two blocks, and only in the min-max game rather than the min-min game. 
For instance, the multi-convexity assumes the convexity of the function concerning each block (coordinate) when the remaining blocks are fixed.%, it is limiting and cannot accommodate nonconvex functions.
On the other hand, the other aforementioned conditions are tailored for objective functions comprising only two blocks. They are particularly defined for min-max type optimizations rather than minimization tasks. 

%From the nonconvexity aspect, there is an increased popularity of the Polyak-{\L}ojasiewicz (PL) condition\footnote{This condition is also referred to as gradient dominant.}.  
The nonconvex optimization realm has seen a growing interest in the gradient dominance condition a.k.a. Polyak-{\L}ojasiewicz (PL) condition. %\footnote{The condition is also known as gradient dominance.}. 
%The PL condition has received considerable focus. 
For instance, in analyzing linear quadratic games \citep{fazel2018global}, matrix decomposition \citep{li2018algorithmic}, robust phase retrieval \citep{sun2018geometric} and training neural networks \citep{hardt2016identity,charles2018stability,liu2022loss}.
This is due to its ability to enable sharp convergence analysis of both deterministic GD and stochastic GD algorithms while being satisfied by a wide range of nonconvex functions.
More formally, a function $f$ satisfies the PL condition if there exists a constant $\mu>0$ such that
\begin{equation}\label{strong_PL}
    \|\nabla f(x)\|^2\geq 2\mu(f(x)-\min_{y\in\mathbb{R}^d}f(y)), \forall x\in\mathbb{R}^d.
\end{equation}
This was first introduced by \cite{polyak1963gradient,lojasiewicz1963topological}, who analyzed the convergence of the GD algorithm under the PL condition and showed its linear convergence to the global minimum. 
This condition can be perceived as a relaxation of strong convexity and as discussed in \citep{karimi2016linear}, it is closely related 
%showed that it is also weaker or equivalent 
to conditions such as weak-strong convexity \!\citep{necoara2019linear}, restricted secant inequality \!\citep{zhang2013gradient} and error bound \!\citep{luo1993error}. 


As mentioned, the PL condition has been extended and applied to optimization problems with multiple coordinates. 
This extension is analogous to generalizing the concept of convexity (concavity) to convex-concavity. 
For instance, the two-sided PL condition was introduced in \citep{yang2020global} for analyzing deterministic and stochastic alternating gradient descent ascent (AGDA) in \textit{min-max games}. 
It is noteworthy that most literature requires convexity or PL condition to establish the last-iterate convergence rate to the NE \citep{scutari2010convex,sohrabi2020survey,jordan2024adaptive}. This, however, may not hold even if the objective function is quadratic. A considerable relaxation is that the function satisfies strong convexity or PL condition when all variables except one are fixed. %Two natural questions arise: 


\textit{Can similar results be achieved by extending the two-sided PL condition to accommodate optimization problems in the form of \eqref{min_problem}, where the objective comprises $n$ coordinates? And is there an algorithm to guarantee convergence at a linear rate in such problems?}

%Furthermore, from \citep{lee2016gradient}, gradient descent with random initialization escapes a NE point almost surely when the point is strictly saddle point.
Furthermore, as highlighted by \citet{lee2016gradient,panageas2016gradient,ahn2022understanding}, GD with random initialization almost surely escapes the NE point when it is a strict saddle point. 
%Also, as simply applying the gradient descent to the potential function tends to approach local minimum if there exists. 
Also, \citet{xu2013block,xu2017globally} require the potential function to be lower-bounded to approach the NE set rather than diverge to infinity. These prompt us to consider the following questions:

\textit{Is it possible to ensure the convergence to the NE set even though it only contains strict saddle points or the function is not lower bounded using first-order GD-based algorithms?}

Motivated by the questions above, we introduce the notion of $n$-sided PL\footnote{We should emphasize that $2$-sided PL and two-sided PL are slightly different conditions as the former is suitable for $\min_{x,y}f(x,y)$ while the latter is for $\min_{x}\max_{y}f(x,y)$.} condition (\cref{PL_condition}), which is an extension to the PL condition and shows that it holds in several well-known nonconvex problems such as $n$-player linear quadratic game, linear residual network, etc. 
It is noteworthy that unlike the two-sided PL condition, which guarantees to converge to the unique Nash Equilibrium (NE) in min-max optimization \citep{yang2020global,chen2022faster}, functions satisfying the $n$-sided PL (even 2-side PL) condition may have multiple NE points (see \cref{sec:def} for examples). However, as we will discuss, the set of stationary points for such functions is equivalent to their NE points. 
Moreover, unlike the two-sided PL condition, which ensures linear convergence of the AGDA algorithm to the NE, the BCD algorithm exhibits varying convergence rates for different functions, all satisfying the $n$-sided PL condition. Similar behavior has been observed with multi-convex functions \citep{xu2017globally,wang2019multi}. Therefore, additional local or global conditions are required to characterize the convergence rate under the $n$-sided PL condition. 

In this work, we study the convergence of first-order GD-based algorithms such as the BCD, and propose different variants of BCD that are more suitable for the class of nonconvex functions satisfying $n$-sided PL condition. We also introduce additional local conditions under which linear convergence can be guaranteed and the convergence to NE still holds even only strict saddle points exist.
%\subsection{Contributions}

% More precisely, our contributions in this work are
% \begin{itemize}
%     \item 

%     \item 

% \end{itemize}




% To study the limited analysis for a function with an arbitrary number of blocks in the minimization problem, we define the $n$-sided Polyak-{\L}ojasiewicz($n$-sided PL) condition, in which for each $i$, $f$ satisfies PL condition while all the other blocks are fixed, for all the blocks and their parameters, i.e.,
% \begin{align}\notag
%      &\|\nabla_{x_i} f(x_i,x_{-i})\|^2\geq 2\mu(f(x_i,x_{-i})-\inf_{y\in\mathbb{R}^{d_i}}f(y,x_{-i})),\\
%      &\forall y\in\mathbb{R}^{d_i},\forall x_{-i},\forall i.
%\end{align}

==> Notations.tex <==
\vspace{-.3cm}
\section{$n$-sided PL Condition}\label{sec:n-pl}
%\vspace{-.3cm}
\textbf{Notations:}
Throughout this work, we use $\|\cdot\|$ to denote the Euclidean norm and the lowercase letters to denote a column vector. In particular, we use $x_{-i}$ to denote the vector $x$ without its $i$-th block, where $i\in[n]:=\{1,...,n\}$.
% and $x=(x_1,...,x_n)\in\mathbb{R}^d$ is a column vector that contains $n$ blocks where $x_i\in\mathbb{R}^{d_i}$ and $d=\sum_{i=1}^n d_i$. 
The partial derivative of $f(x)$ with respect to the variables in its $i$-th block is denoted as $\nabla_{i}f(x):=\frac{\partial}{\partial x_i}f(x_i,x_{-i})$ and the full gradient is denoted as $\nabla f(x)$ that is $(\nabla_{1}f(x),...,\nabla_{n}f(x))$. 
%For a given set $\mathbb{S}$ and a vector $x_{-i}$, we define $\mathbb{S}_{i,x_{-i}}:=\{x_i|(x_i,x_{-i})\in\mathbb{S}\}$ to be the set of $i$-th blocks where $(x_i,x_{-i})$ belongs to  $\mathbb{S}$.
 The distance between a point $x$ and a closed set $\mathbb{S}$ is given by $dist(x, \mathbb{S}):=\inf_{s\in\mathbb S}\|s-x\|$. The uniform sampling between $a$ and $b$ is denoted as $U(a,b)$.

==> Related_Works.tex <==
\vspace{-.3cm}
\subsection{Related Work}
\vspace{-.1cm}

\textbf{Block Coordinate Descent and its variants.} Block coordinate descent (BCD) is an efficient and reliable gradient-based method for optimization problems in \ref{min_problem} which has been used extensively for optimization problems in machine learning \citep{nesterov2012efficiency,allen2016even,zhang2017convergent,zeng2019global,nakamura2021block}. 
Numerous existing works have studied the convergence of BCD and its variants for functions. Most of them require the assumptions of convexity, PL condition, and their extensions \citep{beck2013convergence,hong2017iteration,song2021fast,chen2023global,chorobura2023random}. For instance, \citet{xu2013block, xu2017globally} studied the convergence of BCD for the regularized block multiconvex optimization. They established the last iterate convergence under Kurdyka-{\L}ojasiewicz which might not hold for many functions globally. The authors in \citep{song2021fast} considered the generalized Minty variational problem and applied cyclic coordinate dual averaging with extrapolation to find its solution. Their algorithm is independent of the dimension of the number of coordinates. However, their results rely on assuming the monotonicity of the operators, which is often hard to satisfy. \citet{cai2023cyclic} considered composite nonconvex optimization and applied cyclic block coordinate descent with PAGE-type variance reduced method. They proved linear and non-asymptotic convergence when the PL condition holds, which is not valid for functions with multiple local minima.  

\textbf{PL condition in optimization.} The PL condition was originally proposed to relax the strong convexity in the minimization problem sufficient for achieving the global convergence for first-order methods. For example, \citet{karimi2016linear} showed that the standard GD algorithm admits a linear convergence to minimize an $L$-smooth and $\mu$-PL function. 
To be specific, in order to find an $\epsilon$-approximate optimal solution $\hat{x}$ such that $f(\hat{x})-f^\star\leq\epsilon$, GD requires the computational complexity of the order $O(\frac{L}{\mu}\log\frac{1}{\epsilon})$.
%Despite that many methods such as heavy ball and the accelerated version were guaranteed to achieve linear convergence rate \cite{danilova2020non, wang2022provable}. 
Besides this, different proposed methods, such as the heavy ball method and its accelerated version have been analyzed \citep{danilova2020non,wang2022provable}. 
The authors in \citep{yue2023lower} proved the optimality of GD by showing that any first-order method requires at least $\Omega(\frac{L}{\mu}\log\frac{1}{\epsilon})$ gradient costs to find an $\epsilon$ approximation of the optimal solution. Furthermore, many studies focus on the sample complexity when the objective function has a finite-sum structure, i.e., $f(x)=\frac{1}{n}\sum_{i=1}^{n}f_i(x)$, e.g., \citep{lei2017non, reddi2016stochastic, li2021page, wang2019spiderboost, bai2024complexity}.

In addition to the minimization problem, extensions of the PL condition, such as two-sided conditions, have been proposed to provide convergence guarantees to saddle points for gradient-based algorithms when addressing minimax optimization problems. 
For example, the two-sided PL holds when both $h_y(x):=f(x,y)$ and $h_x(y):=-f(x,y)$ satisfy the PL condition \citep{yang2020global,chen2022faster}, or one-sided PL condition holds when only $h_y(x)$ satisfies the PL condition \citep{guo2020fast,yang2022faster}. 
Various types of first-order methods have been applied to such problems, for example, SPIDER-GDA \citep{chen2022faster}, AGDA \citep{yang2020global}, Multi-step GDA \citep{sanjabi2018solving,nouiehed2019solving}. 
For additional information on the sample complexity of the methods mentioned earlier and their comparisons, see \citep{chen2022faster} and \citep{bai2024complexity}.
%\cite{chen2022faster} and \cite{bai2024complexity} have detailed comparisons for the sample complexity of different methods.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> neurips_2025/1_introduction.tex <==
\section{Introduction}

Optimization problems with nonconvex objectives appear in many applications from computer science and game theory to economics \citep{intriligator2002mathematical} and more recently, in machine learning \citep{jain2017non}, such as training deep neural networks \citep{heaton2018ian} or policy optimization in reinforcement learning \citep{silver2014deterministic}. {
In practice, majority of these applications involve interacting agents whose optimal behavior emerges from solving nonconvex optimization problems.
Despite the notable empirical advancements, there is a lack of understanding of the theoretical convergence guarantees of existing multi-agent methods.
Even the fully cooperative settings remain largely under-explored and constitute one of the current frontiers in machine learning researches. }


{From a game-theoretic perspective, we focus on a multi-agent potential game where the potential function $ f $ captures the aggregate impact of agents' strategies, which is parameterized by $ \{x_i\}_{i=1} ^n$ \citep{monderer1996potential}. Agents aim to optimize the potential function.
%Each agent minimizes $f$ over its variables $x_i$, assuming others' strategies are fixed. 
The most common solution concept for the underlying optimization problem is Nash equilibrium (NE) \citep{nash1950bargaining}. 
Along this line of research, agents are said to be in a Nash equilibrium if no agent can gain by deviating to another policy, provided that the other agents do not deviate. 
We are interested in finding Nash equilibrium $x^\star=(x_1^\star,\cdots,x_n^\star)$ of the nonconvex potential function $f_i(x)$, i.e.,
\begin{equation}\label{min_problem}
        f_i(x_i^\star;x_{-i}^\star)\leq f_i(y_i;x_{-i}^\star),\quad \forall i\in[n], \forall y_i\in\mathbb{R}^{d_i},
\end{equation}
where $x_{-i}^\star$ denotes all blocks except $i$-th block. 
}



%\textcolor{red}{In multi-agent games, the most common solution concept for the underlying optimization problem is Nash equilibrium \cite{XX}(Nash et al., 1950). Despite the notable empirical advancements, there is a lack of understanding of the theoretical convergence guarantees of existing multi-agent methods to the Nash equilibrium. In practice, a majority of the aforementioned applications involve multi-agent interactions. Even the fully cooperative settings remain largely under-explored and constitute one of the current frontiers in AI research. }

%\textcolor{red}{From a game-theoretic perspective, in this work, we focus on is a multi-agent potential game where the potential function $ f $ captures the aggregate impact of agents' strategies, which is parameterized by $ \{x_i\}_{i=1} ^n$ \citep{monderer1996potential}.  Each agent minimizes $f$ over its variables $x_i$, assuming others' strategies are fixed. Along this line of research, agents are said to be in a Nash policy if no agent can improve their reward by deviating to another policy, provided that the other agents do not deviate. We are interested in finding Nash Equilibrium $x^\star=(x_1^\star,\cdots,x_n^\star)$ of the nonconvex potential function $f(x)$, i.e.,}

% However, privacy concerns arise as strategies may reveal sensitive information. In decentralized settings, such as network routing \citet{candogan2010near} or resource allocation \citep{zhang2021potential}, agents optimize independently without full knowledge of $ f $. Furthermore, convergence to an NE is not always stable \citep{carmona2013existence}, as gradient descent may diverge.


% On the other hand, the Gradient Descent (GD) algorithm and its variants are driving the practical success of many machine learning approaches. Naturally, understanding the limits of such GD-based algorithms in the nonconvex setting has become an important avenue of research in recent years \citep{jin2021nonconvex, zhou2018convergence,jordan2023deterministic}.
% Along this line of research, we are interested in finding Nash Equilibrium $x^\star=(x_1^\star,\cdots,x_n^\star)$ of the nonconvex function $f(x)$, i.e.,
% \begin{equation}\label{min_problem}
%         f(x_i^\star;x_{-i}^\star)\leq f(y_i;x_{-i}^\star), \forall y_i\in\mathbb{R}^{d_i},
% \end{equation}
% where $f$ is a continuously differentiable but possibly nonconvex function. The variable $x$ can be partitioned into $n$ blocks $(x_1,...,x_n)$, where $x_i\in\mathbb{R}^{d_i}$ is the $i$-th block and $\sum_{i=1}^n {d_i}=d$. 
% This optimization problem can be viewed as a %general-sum 
% potential game between $n$ players. The objective of $i$-th player is to minimize the function $f(x_i,x_{-i})$ when other players' parameters are denoted by $x_{-i}$.


% From a game-theoretic perspective, this is a multi-agent potential game where the potential function $ f $ captures the aggregate impact of agents' strategies $ \{x_i\}_{i=1}^n $ \citep{monderer1996potential}. 
% Each agent minimizes $f$ over its variables $x_i$, assuming others' strategies are fixed.

When it aims at finding NE, a privacy concern arises as strategies may reveal sensitive information about the agents. In decentralized settings, such as network routing \citet{candogan2010near} or resource allocation \citep{zhang2021potential}, agents optimize independently without full knowledge of $ f $. However, convergence to an NE is not always stable \citep{carmona2013existence}, as gradient descent may diverge.

For a general nonconvex differentiable function $f: \mathbb{R}^d\to\mathbb{R}$, finding its NE is PPAD-complete \citep{daskalakis2009complexity}. 
A straightforward approach to tackle this problem is to introduce additional structural assumptions to achieve convergence guarantees. Within this scope, various relaxations of convexity have been proposed, for example,  weak strong convexity \citep{liu2014asynchronous}, restricted secant inequality \citep{zhang2013gradient}, error bound \citep{cannelli2020asynchronous}, quadratic growth \citep{cui2017quadratic}, etc.  
Recently, there has been a surge of interest in analyzing nonconvex functions with block structure. Multiple assumptions have been analyzed, which are correlated to each block when other blocks are fixed, for example, PL-strongly-concave \citep{guo2020fast}, nonconvex-PL \citep{sanjabi2018solving}, PL-PL \citep{daskalakis2020independent, yang2020global,chen2022faster}, and multi-convex \citep{xu2013block,shen2017disciplined,wang2019multi,wang2022accelerated}. 
For instance, the multi-convexity assumes the convexity of the function with respect to each block (coordinate) when the remaining blocks are fixed.
On the other hand, the other aforementioned conditions are tailored for objective functions comprising only two blocks. They are particularly defined for min-max type optimizations rather than general minimization problems. 

%From the nonconvexity aspect, there is an increased popularity of the Polyak-{\L}ojasiewicz (PL) condition\footnote{This condition is also referred to as gradient dominant.}.  
The nonconvex optimization realm has seen a growing interest in the gradient dominance condition a.k.a. Polyak-{\L}ojasiewicz (PL) condition. %\footnote{The condition is also known as gradient dominance.}. 
For instance, in analyzing linear quadratic games \citep{fazel2018global}, matrix decomposition \citep{li2018algorithmic}, robust phase retrieval \citep{sun2018geometric} and training neural networks \citep{hardt2016identity,charles2018stability,liu2022loss}.
This is due to its ability to enable sharp convergence analysis of both deterministic GD and stochastic GD algorithms while being satisfied by a wide range of nonconvex functions.
More formally, a function $f$ satisfies the PL condition if there exists a constant $\mu>0$ such that
\begin{equation}\label{strong_PL}
    \|\nabla f(x)\|^2\geq 2\mu\big(f(x)-\min_{y\in\mathbb{R}^d}f(y)\big),\quad \forall x\in\mathbb{R}^d.
\end{equation}
This was first introduced by \cite{polyak1963gradient,lojasiewicz1963topological}, who analyzed the convergence of the GD algorithm under the PL condition and showed its linear convergence to the global minimum. 
This condition can be perceived as a relaxation of strong convexity and as discussed in \citep{karimi2016linear}, it is closely related 
%showed that it is also weaker or equivalent 
to conditions such as weak-strong convexity \!\citep{necoara2019linear}, restricted secant inequality \!\citep{zhang2013gradient} and error bound \!\citep{luo1993error}. 


As mentioned, the PL condition has been extended and applied to optimization problems with multiple coordinates. 
This extension is analogous to generalizing the concept of convexity (concavity) to convex-concavity. 
For instance, the two-sided PL condition was introduced in \citep{yang2020global} for analyzing deterministic and stochastic alternating gradient descent ascent (AGDA) in \textit{min-max games}. 
It is noteworthy that most literature requires convexity or PL condition to establish the last-iterate convergence rate to the NE \citep{scutari2010convex,sohrabi2020survey,jordan2024adaptive}. This, however, may not hold even if the objective function is quadratic. A considerable relaxation is that the function satisfies the convexity or PL condition when all variables except one are fixed. 

\begin{shadowboxtext}
\textit{Can similar results be achieved by extending the two-sided PL condition to accommodate problems in the form of \eqref{min_problem}, where the objective comprises $n$ coordinates? And is there an algorithm to guarantee convergence to an NE at a linear rate in such problems?}
\end{shadowboxtext}
Furthermore, as highlighted by \citet{lee2016gradient,panageas2016gradient,ahn2022understanding}, GD algorithm with random initialization almost surely escapes the NE point when it is a strict saddle point. 
Additionally, \citet{xu2013block,xu2017globally} require the potential function to be lower-bounded in order for the iterates to approach the NE set. 
This prompts us to consider the following questions:
\begin{shadowboxtext}
\textit{Is it possible to ensure the convergence to the NE set even though it only contains strict saddle points or the function is not lower bounded using first-order GD-based algorithms?}
\end{shadowboxtext}
Motivated by the above questions, we introduce the notion of $n$-sided PL\footnote{We should emphasize that $2$-sided PL and two-sided PL are slightly different conditions as the former is suitable for $\min_{x,y}f(x,y)$ while the latter is for $\min_{x}\max_{y}f(x,y)$.} condition (\cref{PL_condition}), which is an extension to the PL condition, and show that it holds in several well-known nonconvex problems such as $n$-player linear quadratic game, linear residual network, etc. 
It is noteworthy that, unlike the two-sided PL condition, which guarantees to converge to the unique NE in min-max optimization \citep{yang2020global,chen2022faster}, functions satisfying the $n$-sided PL (even 2-side PL) condition may have multiple NE points (see \cref{sec:def} for examples). However, as we will discuss, the set of stationary points for such functions is equivalent to their NE points. 
Moreover, unlike the two-sided PL condition, which ensures linear convergence of the AGDA algorithm to the NE, the BCD algorithm exhibits varying convergence rates for different functions, all satisfying the $n$-sided PL condition. Similar behavior has been observed with multi-convex functions \citep{xu2017globally,wang2019multi}. Therefore, additional local or global conditions are required to characterize the convergence rate under the $n$-sided PL condition. 

In this work, we study the convergence of first-order GD-based algorithms such as the BCD, and propose different variants of BCD that are more suitable for the class of nonconvex functions satisfying $n$-sided PL condition. 
We show that the convergence to NE still holds when the potential function is not lower bounded and contains only strict saddle points, and introduce additional local conditions under which linear convergence can be guaranteed.





% To study the limited analysis for a function with an arbitrary number of blocks in the minimization problem, we define the $n$-sided Polyak-{\L}ojasiewicz($n$-sided PL) condition, in which for each $i$, $f$ satisfies PL condition while all the other blocks are fixed, for all the blocks and their parameters, i.e.,
% \begin{align}\notag
%      &\|\nabla_{x_i} f(x_i,x_{-i})\|^2\geq 2\mu(f(x_i,x_{-i})-\inf_{y\in\mathbb{R}^{d_i}}f(y,x_{-i})),\\
%      &\forall y\in\mathbb{R}^{d_i},\forall x_{-i},\forall i.
%\end{align}

==> neurips_2025/2_related.tex <==
\vspace{-.3cm}
\subsection{Related Work}
\vspace{-.1cm}

\textbf{Block Coordinate Descent and its variants.} Block coordinate descent (BCD) is an efficient and reliable gradient-based method for optimization problems in \ref{min_problem}, which has been used extensively for optimization problems in machine learning \citep{nesterov2012efficiency,allen2016even,zhang2017convergent,zeng2019global,nakamura2021block}. 
Numerous existing works have studied the convergence of BCD and its variants for functions. Most of them require the assumptions of convexity, PL condition, and their extensions \citep{beck2013convergence,hong2017iteration,song2021fast,chen2023global,chorobura2023random}. For instance, \citet{xu2013block, xu2017globally} studied the convergence of BCD for the regularized block multiconvex optimization. They established the last iterate convergence under Kurdyka-{\L}ojasiewicz, which might not hold for many functions globally. The authors in \citep{song2021fast} considered the generalized Minty variational problem and applied cyclic coordinate dual averaging with extrapolation to find its solution. Their algorithm is independent of the dimension of the number of coordinates. However, their results rely on assuming the monotonicity of the operators, which is often hard to satisfy. \citet{cai2023cyclic} considered composite nonconvex optimization and applied cyclic block coordinate descent with PAGE-type variance reduced method. They proved linear and non-asymptotic convergence when the PL condition holds, which is not valid for functions with multiple local minima.  

\textbf{PL condition in optimization.} The PL condition was originally proposed to relax the strong convexity in the minimization problem sufficient for achieving the global convergence for first-order methods. For example, \citet{karimi2016linear} showed that the standard GD algorithm admits a linear convergence to minimize an $L$-smooth and $\mu$-PL function. 
To be specific, in order to find an $\epsilon$-approximate optimal solution $\hat{x}$ such that $f(\hat{x})-f^\star\leq\epsilon$, GD requires the computational complexity of the order $O(\frac{L}{\mu}\log\frac{1}{\epsilon})$.
%Despite that many methods such as heavy ball and the accelerated version were guaranteed to achieve linear convergence rate \cite{danilova2020non, wang2022provable}. 
Besides this, different proposed methods, such as the heavy ball method and its accelerated version, have been analyzed \citep{danilova2020non,wang2022provable}. 
The authors in \citep{yue2023lower} proved the optimality of GD by showing that any first-order method requires at least $\Omega(\frac{L}{\mu}\log\frac{1}{\epsilon})$ gradient costs to find an $\epsilon$ approximation of the optimal solution. Furthermore, many studies focus on the sample complexity when the objective function has a finite-sum structure, i.e., $f(x)=\frac{1}{n}\sum_{i=1}^{n}f_i(x)$, e.g., \citep{lei2017non, reddi2016stochastic, li2021page, wang2019spiderboost, bai2024complexity}.

In addition to the minimization problem, extensions of the PL condition, such as two-sided conditions, have been proposed to provide convergence guarantees to saddle points for gradient-based algorithms when addressing minimax optimization problems. 
For example, the two-sided PL holds when both $h_y(x):=f(x,y)$ and $h_x(y):=-f(x,y)$ satisfy the PL condition \citep{yang2020global,chen2022faster}, or one-sided PL condition holds when only $h_y(x)$ satisfies the PL condition \citep{guo2020fast,yang2022faster}. 
Various types of first-order methods have been applied to such problems, for example, SPIDER-GDA \citep{chen2022faster}, AGDA \citep{yang2020global}, Multi-step GDA \citep{sanjabi2018solving,nouiehed2019solving}. 
For additional information on the sample complexity of the methods mentioned earlier and their comparisons, see \citep{chen2022faster} and \citep{bai2024complexity}.
%\cite{chen2022faster} and \cite{bai2024complexity} have detailed comparisons for the sample complexity of different methods.



==> neurips_2025/3_definitions.tex <==
\vspace{-.3cm}
\section{$n$-sided PL Condition}\label{sec:n-pl}
\vspace{-.3cm}
\textbf{Notations:}
Throughout this work, we use $\|\cdot\|$ to denote the Euclidean norm and the lowercase letters to denote a column vector. In particular, we use $x_{-i}$ to denote the vector $x$ without its $i$-th block, where $i\in[n]:=\{1,...,n\}$.
% and $x=(x_1,...,x_n)\in\mathbb{R}^d$ is a column vector that contains $n$ blocks where $x_i\in\mathbb{R}^{d_i}$ and $d=\sum_{i=1}^n d_i$. 
The partial derivative of $f(x)$ with respect to the variables in its $i$-th block is denoted as $\nabla_{i}f(x):=\frac{\partial}{\partial x_i}f(x_i,x_{-i})$ and the full gradient is denoted as $\nabla f(x)$ that is $(\nabla_{1}f(x),...,\nabla_{n}f(x))$. 
%For a given set $\mathbb{S}$ and a vector $x_{-i}$, we define $\mathbb{S}_{i,x_{-i}}:=\{x_i|(x_i,x_{-i})\in\mathbb{S}\}$ to be the set of $i$-th blocks where $(x_i,x_{-i})$ belongs to  $\mathbb{S}$.
 The distance between a point $x$ and a closed set $\mathbb{S}$ is given by $dist(x, \mathbb{S}):=\inf_{s\in\mathbb S}\|s-x\|$. The uniform sampling between $a$ and $b$ is denoted as $U(a,b)$. The set of all functions that are $n$-th order differentiable is $C^n$. The ball centered at $x$ with radius $r$ is $\mathcal{B}(x,r)$.

\vspace{-.1cm}
\subsection{Definitions and Assumptions}\label{sec:def}


In this paper, we assume the function $f(x):$ $\mathbb{R}^d\to\mathbb{R}$ belongs to $C^1$, i.e., it is continuously differentiable. Furthermore, we assume it has a Lipschitz gradient.

\begin{assumption}[Smoothness]\label{L_Lip}
We assume the $L$-Lipschitz continuity of the derivative $\nabla f(x)$,
\begin{equation*}
    \|\nabla f_i(x)-\nabla f_i(y)\|\leq L\|x-y\|, \forall i,x, y
\end{equation*}
where $L>0$ is a constant. In this case, $f(x)$ is also called $L$-smooth.
\end{assumption}

\begin{assumption}[Lower bounded]\label{lower-bounded}
The function $f(x)$ is lower bounded, i.e. $\inf_{x\in\mathbb{R}^{d}} f(x)>-\infty$.
\end{assumption}


We now define two notions of optimality for $\min_x f(x_1,...,x_n)$; NE and Stationary point. 
%One of the notions of optimality is Nash Equilibrium, at which $x_i^{\star}$ is an optimal solution to the function $f_i(x)=f(x,x_{-i}^\star)$ for all $i\in[n]$.

\begin{definition}[Nash Equilibrium (NE)]
 Point $x^\star=(x_1^\star,...,x_n^\star)$ is called a Nash Equilibrium of function $f(x)$ if 
 \begin{equation*}
     f_i(x_{i}^\star,x_{-i}^\star)\leq f_i( x_{i},x_{-i}^\star), \quad \forall i\in[n], \forall x_i\in\mathbb{R}^{d_i}.
 \end{equation*}
The set of all NE points of $f(x)$ is denoted by $\mathcal{N}(f)$.
\end{definition}
The other notion, the stationary point, is related to the first-order condition of optimality and also relevant for studying gradient-based algorithms.

%\begin{definition}[Stationary Point]
%    A point $x^\star$ is a stationary point if
%    \begin{equation}
%        \nabla f(x^\star)=0.
%    \end{equation}
%\end{definition}
\begin{definition}[$\varepsilon$-Stationary point]
    Point $\tilde x=(\tilde x_1,...,\tilde x_n)$ is called an $\varepsilon$-stationary point of $f(x)$ if 
    $
    \|\nabla f(\tilde x)\|\leq \varepsilon.
    $
    When $\varepsilon=0$, the point $\tilde x$ is called a stationary point. We denote the set of all $\varepsilon$-stationary points and the set of all stationary points of $f(x)$ by $\mathcal{S}_\varepsilon(f)$ and $\mathcal{S}(f)$, respectively.
\end{definition}
For general nonconvex minimization problems, the above two notions are not necessarily equivalent, i.e., a stationary point may not be an NE. 
Nevertheless, for the remainder of this work, we assume that the objective function $f$ has at least one NE, i.e., $\mathcal{N}(f)\neq \emptyset$. We also assume that $\arg\min_{x_i\in\mathbb{R}^{d_i}}f(x_i,x_{-i})$ is non-empty for any $i\in[n]$ and $x_{-i}$, i.e., there exists a best response to every $x_{-i}$. Note that this is not a limiting assumption given that the function is lower bounded. 
Below, we formally introduce the $n$-sided PL condition for the function $f(x)$.

\begin{shadowboxtext}
\begin{definition}[$n$-sided PL Condition]\label{PL_condition}
We say $f(x)=f(x_1,...,x_n)$ satisfies $n$-sided $\mu$-PL condition if there exists a positive constant $\mu>0$ such that for all $x\in\mathbb{R}^{d}, i\in[n]$
\begin{align}\label{eq:n-sided}
\|\nabla_{i}f_i(x_i,x_{-i})\|^2\geq 2\mu\big(f_i(x_i,x_{-i})-f_{i,x_{-i}}^\star\big), 
\end{align}   
\vspace{-.1cm}
where $f_{i,x_{-i}}^\star:=\min_{y_i} f_i(y_i,x_{-i})$.    
\end{definition}
\end{shadowboxtext}

It is worth noting that the $n$-sided PL condition does not imply convexity or the gradient dominance (PL) condition. It is an extension to the PL condition, as when $f$ is independent of $x_{-i}$, 
then $f$ satisfies the PL condition. Moreover, it is considerably weaker than multi-strong convexity.
Nevertheless, under the $n$-sided PL condition, the set of stationary points and the NE set are equivalent.
%\textcolor{red}{delete} For instance, the set of stationary points and the NE set of $f_0$ in Figure \ref{fig:example1} is $\{(-1,-1), (1,1), (0,0)\}$. All proofs are in the Appendix \ref{sec:proofs}.
\begin{lemma}\label{SP_equal_NE}
If $f(x_1,...,x_n)$ satisfies the $n$-sided PL condition, then $\mathcal{S}(f)=\mathcal{N}(f)$
\end{lemma} 
All proofs are in the Appendix \ref{sec:proofs}.
%It is also important to emphasize that, unlike the $n$-sided PL, the two-sided PL condition is defined such that the right-hand side of \eqref{eq:n-sided} is the difference between the function and its minimum for one coordinate while for the other coordinate it is the difference between the function and its maximum. As a consequence, under the two-sided condition, the stationary points are also global minimax points.
It is noteworthy that, unlike the two-sided PL condition, under the $n$-sided PL condition in \cref{PL_condition}, it is no longer possible to ensure that the NE is unique. In fact, there could be multiple NEs with different function values. For example, consider the functions $f_0(x,y)$ and $f(x,y)$ illustrated in Figure \ref{fig:example1}. As shown in Appendix \ref{app:example}, both functions are $2$-sided PL, but their set of NE and the set of minimum points are not equivalent. 
In particular, both functions have three NE points while $f_0(x,y)$ has two global minimums and a saddle point, and $f(x,y)$ has a local minimum, a global minimum, and a saddle point. 
\begin{figure}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=0.44\linewidth,,height=2cm]{example1.jpg}
         %\caption{Function $f_0(x,y)=(x-1)^2(y+1)^2+(x+1)^2(y-1)^2$.}
         \label{fig:y equals x}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[width=0.42\linewidth,,height=2cm]{Example2.png}
         %\caption{Function $f(x,y)=(x-1)^2(y+1)^2+(x+1)^2(y-1)^2+\exp(-(y-1)^2)$.}
         \label{fig:three sin x}
     \end{subfigure}
        \caption{Left is function \begin{small}$f_0(x,y)\!=\!(x-1)^2(y+1)^2\!+\!(x+1)^2(y-1)^2$\end{small} and right is function \begin{small}$f(x,y)=f_0(x,y)+\exp(-(y-1)^2)$\end{small}.}
        \label{fig:example1}
\end{figure}

















==> neurips_2025/6_algorithms.tex <==
\vspace{-.2cm}
\section{Algorithms and Convergence Analysis}\label{sec:algs}

In this section, we first study the BCD algorithm for finding a stationary point of \eqref{min_problem} under the $n$-sided PL condition. 
Afterward, we propose different variants of BCD algorithms that can provably achieve better convergence rates. 

The BCD algorithm is a coordinate-wise approach that iteratively improves its current estimate by updating a selected block coordinate using the first-order partial derivatives until it converges. 
% \begin{wrapfigure}{r}{0.45\textwidth}
% \begin{minipage}{0.45\textwidth}
% \vspace{-.3cm}
% \begin{algorithm}[H]
% \caption{Cyclic Block Coordinate Descent (BCD)}\label{alg:BCD}
% \begin{algorithmic}
%    \STATE {\bfseries Input:} initial point $x^0=(x_1^0,...,x_n^0)$, learning rates $\alpha$
%    \FOR{$t=1$ {\bfseries to} $n$}
%    \FOR{$i=1$ {\bfseries to} $n$}
%    \STATE $x_i^t=x_i^{t-1}-\alpha\nabla_{i}f(x_{1:i-1}^t,x_{i:n}^{t-1})$
%    \ENDFOR
%    \ENDFOR
% \end{algorithmic}
% \end{algorithm}
%   \end{minipage}
% \vspace{-.2cm}
% \end{wrapfigure}
Depending on how the coordinates are chosen, various types of BCD algorithms can be devised.
For example, coordinates can be selected uniformly at random for \textit{random BCD}, or in a deterministic cyclic sequence for \textit{cyclic BCD}.
Algorithm \ref{alg:BCD} in the Appendix presents the \textit{cyclic BCD} with {learning rates} $\alpha$. 
Moreover, to update the $i$-th block at the $t$-th iteration, it employs $\nabla_{i}f(x_{1:i-1}^t,x_{i:n}^{t-1})$, where $(x_{1:i-1}^t,x_{i:n}^{t-1})$ denotes the latest estimated point, which is $(x_1^t,...,x_{i-1}^t,x_i^{t-1},...,x_n^{t-1})$.
The next result shows that when the iterates of the BCD are bounded, the output converges to the NE set. 

\begin{theorem}\label{bounded_to_converge}
Under the Assumptions \ref{L_Lip} and \ref{lower-bounded}, by applying BCD algorithm, if $f(x)$ satisfies $n$-sided PL condition, the iterates $\{x^t\}$ are bounded and the learning rates $\alpha\leq\frac{1}{L}$, then $\lim_{t\to+\infty}dist\big(x^t,\mathcal{N}(f)\big)=0$.
\end{theorem}

%\textcolor{red}{need to delete}The above result ensures the convergence of BCD to the NE set, but it does not necessarily indicate whether the output converges to a point within the NE set. The convergence to a point within the NE set can be established if every point in the NE set is isolated, e.g., $f_0$ and $f$ in Figure \ref{fig:example1}.

%\begin{theorem}\label{isolated_point}\textcolor{red}{maybe delete this}
%Under the assumptions of \cref{bounded_to_converge}, if $\mathcal{N}(f)$ is the union of isolated points, i.e., there exists $\eta>0$, such that $\min_{\substack{y\neq z\in\mathcal{N}(f)}}\|y-z\|\geq\eta$, then $\{x^t\}$ converges to a point in $\mathcal{N}(f)$.
%\end{theorem}


\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-.4cm}
\begin{minipage}{0.4\textwidth}
\centering
    \includegraphics[width=6cm,height=3.3cm]{bcd_low.png}
      \vspace{-.4cm}
    \caption{The BCD algorithm applied to functions $f_1(x,y)$ and $f_2(x,y)$. The y-axis is in log scale, thus the BCD demonstrates linear convergence for $f_2$.}\label{bcd_low}
\end{minipage}
    \vspace{-.4cm}
\end{wrapfigure}
It is noteworthy that, following the results of \citet{lee2016gradient,lee2019first,panageas2016gradient,ahn2022understanding}, when the function is smooth and the initial points are chosen randomly, the BCD algorithm avoids strict saddle points in the NE set almost surely. See the Appendix \ref{sec:almostsurely} for formal statements and proofs. 

Although the above results ensure the convergence of BCD when the function is lower bounded, they do not specify the last-iterate convergence rate. 
Unlike the two-sided PL condition that leads to linear convergence of AGDA to the min-max, the $n$-sided PL condition does not necessarily lead to any specific convergence rate of the BCD. 
To demonstrate this phenomena, we consider two $2$-sided PL functions: $f_1(x,y)=(x+y)^2+\exp(-1/(x-y)^2)$ for $(x,y)\neq (0,0)$ and zero otherwise and $f_2(x,y)=(x+y)^2$. 
We applied the BCD algorithm to both these functions with constant learning rates to find their NE points with random initializations. 

As it is illustrated in Figure \ref{bcd_low}, the BCD converges linearly for the function $f_2$ while it converges sub-linearly for $f_1$.
This example shows that characterizing the convergence rate of the BCD algorithm under the $n$-sided PL condition and the smoothness might not be feasible, and further assumptions on the function class are required. 
Next, we study one such assumption that holds for a large class of non-convex functions and could characterize the convergence rate of random BCD.


\subsection{ Convergence of random BCD under an additional assumption} 
To introduce our additional assumption, we need to define the average of the best responses, denoted by $G_F(x)$, which plays a central role in analyzing the convergence of coordinate-wise algorithms. 
\begin{align}\label{eq:G_Function}
    G_F(x):=\frac{1}{n}\sum_{i=1}^n f_i(x^*_i(x),x_{-i}),
\end{align}
where $x^*_i(x)$ denotes the best response to $x_{-i}$ that is the closest to $x_i$, i.e., $x^*_i(x)\in\arg\min_{y_i}\{\|y_i-x_i\|:\ (y_i,x_{-i})\leq f(z_i,x_{-i}),\forall z_i\}$. 
It is straightforward to see that $f(x)-G_F(x)\geq 0$ for all $x$.
Moreover, if $x^*\in\mathcal{N}_f$, then $f(x^*)=G_F(x^*)$. Conversely, if $f(x^*)-G_F(x^*)=0$, then $f(x^\star)=\min_{x_i}f(x_i,x_{-i}^\star)$, $\forall i$, which implies $x^\star\in\mathcal{N}_f$. 
 
\begin{lemma}
    $x^\star$ is a NE if and only if $f(x^\star)-G_F(x^\star)=0$.
\end{lemma}

Thus, $f(x) - G_F(x)$ serves as an indicator of whether $x$ is an NE. Using this indicator, we show that the random BCD algorithm achieves a linear convergence rate under an additional assumption.
%In the next result, we show that $G_F(x)$ is also both differentiable and smooth under the $n$-sided PL condition. 
%\begin{lemma}\label{G_smooth}
%    If $f(x)$ satisfies $n$-sided $\mu$-PL and satisfies \cref{L_Lip}, then $G_F(x)$ is $L'$-smooth, where $L':=L+\frac{L^2}{\mu}$.
%\end{lemma}
%Note that if function $f(x)$ is $L$-smooth and $n$-sided $\mu$-PL, then $L\geq \mu$ (see Appendix \ref{sec:tech})
\begin{theorem}\label{convergence_ideal_kt0}
Suppose $f(x)$ is an $n$-sided $\mu$-PL function satisfying \cref{L_Lip} such that $\langle\nabla G_F(x),\nabla f(x)\rangle\leq\kappa \|\nabla f(x)\|^2$, where $\kappa<1$, then random BCD with $\alpha^t:=\alpha\leq\frac{2(1-\kappa)}{2(L+\frac{L^2}{\mu})+(1+\kappa)L}$ achieves linear convergence rate, i.e., 
\begin{small}
\begin{equation*}
    \mathbb{E}[f(x^{t+1})-G_F(x^{t+1})] \leq \big(1-\frac{\mu\alpha(1-\kappa)}{2}\big)\ \mathbb{E}[f(x^t)-G_F(x^t)].
\end{equation*}
\end{small}
The expectation is taken over the randomness inherent in the procedure for selecting coordinates.
\end{theorem}

%Below, we introduce an additional assumption on $f$ under which the random BCD algorithm achieves a linear convergence rate. This is about how the gradients of $f$ and $G_F$ are aligned  
%\begin{assumption}\label{ass:new}\textcolor{red}{maybe delete this}
%For a given set of points $\{x^1,x^2,...\}$, there exists $0\leq\kappa<1$ such that for all $\tau$,
%\begin{align}\label{eq:additional_as}
%    \langle\nabla G_F(x^\tau),\nabla f(x^\tau)\rangle\leq\kappa \|\nabla f(x^\tau)\|^2.
%\end{align}
%\end{assumption}
It is straightforward to show that functions $f_2$ in Figure \ref{bcd_low} and $f_0$ in Figure \ref{fig:example1} satisfy $\langle\nabla G_F(x),\nabla f(x)\rangle<\|\nabla f(x)\|^2$ for all points within $\mathbb{R}^2$ and $\{(x,y)\!:\! |x|\!>\!0.75, |y|\!>\!0.75\}$, respectively. Note that this set contains both local minimums of $f_0$. 
%\textcolor{red}{delete this GD discussion} Similar convergence rate can be achieved using GD algorithm, i.e., $x^t=x^{t-1}-\alpha^t\nabla f(x^{t-1})$. See Appendix \ref{app:gd}.  Under the \cref{ass:new}, the linear convergence of  $\mathbb{E}[f-G_F]$ is guaranteed using random BCD. This assumption is correlated with the local strong convexity. 

To show that the additional assumption in Theorem \ref{convergence_ideal_kt0} is not restrictive, we prove that around every isolated minimum of a locally strongly convex and smooth function, this assumption holds on average for all iterates of the GD algorithm. 

\begin{theorem}\label{thm:avergae_case3}
Let $x^\star$ denotes the isolated local minimum in a neighborhood $U$ and $G_F$ exists, then there exists a radius $r>0$ s.t. $\forall x_0\in\mathcal{B}(x^\star,r)\subseteq U$ and by following the dynamics $\dot{r}(t)=-\nabla f(x)|_{x=r(t)}$, $r(0)=x_0$, we have
\begin{small}
\begin{equation*}
  \int_0^{+\infty}\!\!\!\! \langle\nabla G_F(x), \nabla f(x)\rangle\big|_{x=r(t)} dt \leq\! \! \int_0^{+\infty}\!\!\!\!\!\! \|\nabla f(x)\|^2\big|_{x=r(t)} dt.
\end{equation*}
\end{small}
Furthermore, if $\nabla^2 f(x^\star)\!\succ\! 0$, $\nabla^2\!f$ is continuous, and $f$ is $L$-smooth, then there exists $0\!\leq\! \kappa\!<\!1$, s.t.
\begin{small}
\begin{equation*}
        \int_0^{+\infty}\!\!\!\!\langle\nabla G_F(x), \nabla f(x)\rangle\big|_{x=r(t)} dt
        \leq\!\kappa\!\!\int_0^{+\infty}\!\!\!\!\|\nabla f(x)\|^2\big|_{x=r(t)}dt.
\end{equation*}       
\end{small}
\vspace{-.3cm}
\end{theorem}



%Applying the Cauchy-Schwarz inequality leads to a stronger assumption than \cref{ass:new} that is there exists $0\leq\kappa<1$, such that $\|\nabla G_F(x^t)\|\leq\kappa \|\nabla f(x^t)\|$. On the other hand, the following result shows that $\|\nabla G_F\|$ is always bounded from above by $\|\nabla f\|$ for $n$-sided PL function $f$, but with a constant greater than one. The constant being greater than one in this result is a consequence of the proof's construction. Thus, for instance, if the function $f$ is such that this constant is less than one for the iterates of the random BCD, then linear convergence can be guaranteed by \cref{convergence_ideal_kt0}. This is indeed the case for functions such as $f_0$ and the linear residual network problem (see Section \ref{sec:applications}). 
%\begin{lemma}\label{G_deri_bound}
%   \textcolor{red}{maybe delete this}For an $n$-sided $\mu$-PL function $f(x)$ satisfying \cref{L_Lip}, let $C_{f}:=\frac{L}{\sqrt{n}\mu}+1$, then $\|\nabla G_F(x)\|\leq C_{f}\|\nabla f(x)\|$, for all $x$.
%\end{lemma}


%\subsection{Convergence with the exact best responses but without additional assumption}

\subsection{Adaptive random BCD with the knowledge of exact best responses}

%  \begin{wrapfigure}{r}{0.53\textwidth}
%  \vspace{-.7cm}
% \begin{minipage}{0.53\textwidth}
\begin{algorithm}[H]
   \caption{Ideal Adaptive random BCD (IA-RBCD)}
\begin{algorithmic}\label{arbcd_ideal}
   \STATE {\bfseries Input:} initial point $x^0=(x_1^0,...,x_n^0)$, $T$, learning rates $\alpha$, $0\leq\gamma<1$ and $C>0$
   \FOR{$t=0$ {\bfseries to} $T-1$}
   \STATE sample $i^t$ uniformly from $\{1,2,...,n\}$
   %\STATE compute $\nabla G(x^t)=\frac{1}{n}\sum_{l=1}^n\nabla \min_{x_i}f(x_i,x_{-i}^{t})$
   \IF{$\langle\nabla G_F(x^t),\nabla f(x^t)\rangle \leq \gamma \|\nabla f(x^t)\|^2$}
   \STATE $k^t=0$ \hfill\texttt{:Case 1:}
   \ELSIF{$\frac{(\|\nabla G_F(x^t)\|^2-\langle\nabla f(x^t),\nabla G(x^t)\rangle)^2}{\langle\nabla f(x^t),\nabla G(x^t)\rangle^2}>C$}
   \STATE $k^t=-2+\frac{\langle\nabla f(x^t),\nabla G_F(x^t)\rangle}{\|\nabla G_F(x^t)\|^2}$ \hfill\texttt{:Case 2:}
   \ELSE   \STATE $k^t=-1$ \hfill\texttt{:Case 3:}
   \ENDIF
   \STATE $x_{i^t}^{t+1}=x_{i^t}^{t}-\alpha(\nabla_{{i^t}}f(x^{t})+k^t\nabla_{i^t}G_F(x^t)),$ $x_{i}^{t+1}=x_{i}^{t}$\quad if\quad $i\neq i^t$
   \ENDFOR
   %\STATE {\bfseries Output:} $x^{T}=(x_1^{T},...,x_n^{T})$
\end{algorithmic}
\end{algorithm}
% \end{minipage}
%  \vspace{-.5cm}
% \end{wrapfigure}
As we discussed earlier, the BCD algorithms may demonstrate different convergence rates in general. 
Thus, our objective in the remainder of this section is to develop variants of the random BCD and GD algorithms so that close to linear convergence is still achievable. 
%To do so, we design algorithms that iteratively update by considering the best responses, $\{x^*_i(x^t)\}$, at each iteration $t$.
To this end, we propose algorithms that, at each iteration $t$, update the variables based on the best responses $\{x^*_i(x^t)\}$.
We initially propose an algorithm that presumes access to the exact values of the best responses at each iteration. 
Subsequently, we refine this assumption by integrating a sub-routine into the proposed algorithm capable of approximating the best responses.
% For the sake of simplicity and space, we describe our block coordinate variants here and the GD variants and their convergence analysis are presented in the Appendix \ref{sec:adaptive_alg}. 
To present our results, we need the following definition.
\begin{definition} [$(\theta,\nu)$-PL condition]
 The function $f$ with $\min_x f(x)=0$ satisfies $(\theta,\nu)$-PL condition iff there exists $\theta \in[1,2)$ and $\nu>0$ such that $\|\nabla f(x)\|^\theta \geq(2 \nu)^{\theta / 2} f(x). \quad$    
\end{definition}
It has been proved by \citet{lojasiewicz1963topological} that for any $C^1$ analytic function, there exists a neighborhood $U$ around the minimizer where $(\theta,\nu)$-PL condition is satisfied.


Algorithm \ref{arbcd_ideal} presents the steps of our modified version of the random BCD. In this algorithm, instead of updating along the direction of $-\nabla_{i^t} f(x)$, where $i^t$ denotes the chosen coordinate at iteration $t$, a linear combination of $\nabla_{{i^t}}f(x)$ and $\nabla_{i^t}G_F(x)$ is used to refine the updating directions.
The coefficient of this linear combination, \(k^t\), is adaptively selected based on the current estimated point. 
It is important to mention that $\nabla G_F(x)$ can be computed using the gradient of $f$ at the best responses,
\begin{small}
\vspace{-.2cm}
\begin{align}\label{eq:gradient_g}
    \nabla G_F(x)=\frac{1}{n}\sum_{i=1}^n\nabla f\big(x^*_i(x), x_{-i}\big).
\end{align}
\end{small}
As it is shown in Appendix \ref{proof:G_smooth}, this function is $L'$-smooth, where $L'=L+\frac{L^2}{\mu}$.
\begin{shadowboxtext}
\begin{theorem}\label{convergence_ideal}
\vspace{-.2cm}
For $n$-sided $\mu$-PL function $f(x)$ satisfying \cref{L_Lip}, by applying \cref{arbcd_ideal}, 

\begin{itemize}[leftmargin=8pt]
\item in Case 1 with $\alpha\!\leq\!\frac{2(1-\gamma)}{2L'+(1+\gamma)L}$, we have 
\begin{small}
$\mathbb{E}[f(x^{t+1})\!-\!G_F(x^{t+1})|x^t]\! \leq\! \big(1\!-\!\frac{\mu\alpha(1-\gamma)}{2}\big)(f(x^t)\!-\!G_F(x^t)),$
\end{small}

\item in Case 2 with $\alpha\!\leq\min\{\frac{1}{2(L+L')},\frac{C}{2(L+L')}\}$, we have
\begin{small}
$
\mathbb{E}[f(x^{t+1})\!-\!G_F(x^{t+1})|x^t]\!\leq\!\! \big(1\!-\!\!\frac{(L+L')\mu\alpha^2}{2}\big)\ (f(x^t)\!-\!G_F(x^t)),
 $
\end{small}

\item in Case 3 with $\alpha\!\leq\!\frac{1}{L+L'}$, $f-G_F$ is non-increasing. Furthermore, if $f-G_F$ satisfies $(\theta,\nu)$-PL condition and case 3 are satisfied from iterates $t$ to $t+k$, we have
\begin{small}
\begin{equation*}
    \mathbb{E}[f(x^{t+k})-G_F(x^{t+k})|x^t]=\mathcal{O}\Big(\frac{f(x^{t})-G_F(x^{t})}{k^{\frac{\theta}{2-\theta}}}\Big).    
\end{equation*}
\end{small}
\end{itemize}
\vspace{-.3cm}
\end{theorem}
\end{shadowboxtext}

The exact constant terms are provided in the proof. 
It is crucial to highlight that BCD requires \cref{lower-bounded} to converge to the NE \citep{xu2013block} and almost surely avoids strict saddle points \citep{lee2016gradient}. However, this result shows that IA-RBCD converges to the NE, irrespective of this condition.
Additionally, based on this result, IA-RBCD in \ref{arbcd_ideal} demonstrates a linear rate for two out of three cases and a sub-linear rate for the third case. Next, we show that even if the third case occurs frequently, linear convergence is still guaranteed by IA-RBCD. 
Determining precisely how often case 3 occurs requires additional local properties of the NEs. For example, if the function is locally strongly convex around the NE, case 3 will not occur.

% \begin{theorem}\label{case_many_enough}
%     Under the assumptions of \cref{convergence_ideal}, by applying Algorithm \ref{arbcd_ideal} for $t$ iterations and denoting the number of iterations, it visits Case 3 by $b(t)$($\leq t$), if
%     $ B:=\lim\sup_{t\to +\infty} b(t)/t<1$,
%     then $\forall\epsilon$ such that $0<\epsilon< 1-B$, there exists $\hat{t}$ such that for all $t\geq \hat{t}$,
%     \begin{equation*}
%         \mathbb{E}[f(x^t)-G_F(x^t)]\leq c^{t}\cdot(f(x^0)-G_F(x^0)),
%     \end{equation*}
%      where $c\!:=\!\big(\min\{1-\frac{\mu\alpha(1-\kappa)}{2},1-\frac{(L+L')\mu\alpha^2}{2}\}\big)^{1-B-\epsilon}\!\!<1$.
% \end{theorem}

\begin{shadowboxtext}
\begin{theorem}\label{case_many_enough}
    Under the assumptions of \cref{convergence_ideal}, by applying Algorithm \ref{arbcd_ideal} for $t$ iterations and denoting the number of iterations it visits Case 3 by $b(t)$, if
    $ B:=\lim\sup_{t\to +\infty} b(t)/t<1$,
    then there exists $0<c_B<1$ and $\hat{T}_B$ such that for all $t\geq \hat{T}_B$,
    \begin{equation*}
        \mathbb{E}[f(x^t)-G_F(x^t)]\leq c_B^{t}\cdot(f(x^0)-G_F(x^0)).
    \end{equation*}
\end{theorem}
\end{shadowboxtext}

We empirically verify the rarity of Case 3 in Section \ref{sec:applications} across several well-known problems.
In the following theorem, we demonstrate that as $\gamma \to 1$ and $C \to 0$, the measure of non-NE points that fail to satisfy case 1 and case 2 converges to zero. Furthermore, when the iterates fall into case 3, $f-G_F$ is small at those iterates which indicates that a good approximation of an NE is already achieved. 
As a consequence, by choosing hyperparameters $\gamma$ and $C$ close to one and zero, respectively, we can achieve close to linear convergence rate.

\begin{shadowboxtext}
\begin{theorem}\label{thm:measure}
    If $f(x)$ satisfies the assumption of \cref{convergence_ideal}, then, by defining $S(\gamma, C)$ to be the set of non-NE points that do not satisfy case 1 and case 2, we have
    \begin{equation*}
        \lim_{\gamma\to 1, C\to 0} |S(\gamma,C)|=0,
    \end{equation*}
    where $|S(\gamma, C)|$ denotes the measure of the set $S(\gamma, C)$. Moreover, if $S(\gamma,C)$ is non-empty, then
        $\lim_{\gamma\to 1, C\to 0} \max_{x\in S(\gamma, C)}f(x)-G_F(x)=0$.
\end{theorem}
\end{shadowboxtext}



%\vspace{-.1cm}
%\subsection{Convergence without the exact best responses and the additional assumption}
\subsection{Adaptive random BCD without the knowledge of exact best responses}

Evaluating $G_F$ at a given point requires knowledge of the best responses at that point. Often, these best responses are not known a priori, and they have to be computed at each iteration.  
Fortunately, since in our study, $f$ satisfies the $n$-sided PL condition, the best responses can be efficiently approximated by applying the GD algorithm with the partial gradients as a sub-routine.
Algorithm \ref{sub-routine} in the Appendix presents the steps of this sub-routine, and Algorithm \ref{arbcd_practical} shows the steps of our adaptive random BCD algorithm. 
%The main difference between algorithms \ref{arbcd_ideal} and \ref{arbcd_practical} is that at every iteration, A-RBCD approximates the best responses function by gradient descent. 
According to the next result, the number of steps for approximating $G_F$, $T'$, only depends on the function parameters, and it is independent of the final precision of $f-G_F$. 
%\textcolor{red}{maybe also simplify this}
%In other words, to achieve $f(x)-G_F(x)\leq \epsilon$, we only need $O(\log(1/\epsilon))$ steps of computing gradient.

%  \begin{wrapfigure}{r}{0.53\textwidth}
% \vspace{-.7cm}
% \begin{minipage}{0.53\textwidth}
\begin{algorithm}[H]
   \caption{Adaptive random BCD (A-RBCD)}
\begin{algorithmic}\label{arbcd_practical}
   \STATE {\bfseries Input:} initial point $x^0=(x_1^0,...,x_n^0)$, $T, T'$,  learning rates $\alpha$, $\beta$, $0<\gamma<1$ and $C>0$
   \FOR{$t=0$ {\bfseries to} $T-1$}
   \STATE sample $i^t$ uniformly from $\{1,2,...,n\}$
   \STATE $y^{t,T'}=$ABR$(x^{t}, T', \beta)$ \hfill \texttt{:Algorithm \ref{sub-routine}}
   \STATE compute $\tilde\nabla G_F(x^t)=\frac{1}{n}\sum_{l=1}^n\nabla f(y_l^{t,T'},x_{-l}^{t})$
   \IF{$\langle\tilde\nabla G_F(x^t),\nabla f(x^t)\rangle\leq (\gamma-\gamma\frac{\alpha^{3}}{13}) \|\nabla f(x^t)\|^2$}
   \STATE $\tilde k^t=0$ \hfill\texttt{:Case 1:}
   \ELSIF{$\frac{(\|\tilde\nabla G_F(x^t)\|^2-\langle\nabla f(x^t),\tilde\nabla G_F(x^t)\rangle)^2}{\|\tilde\nabla G_F(x^t)\|^4}>C$ }
   \STATE $\tilde k^t=-2+\frac{\langle\nabla f(x^t),\tilde\nabla G_F(x^t)\rangle}{\|\tilde\nabla G_F(x^t)\|^2}$\hfill\texttt{:Case 2:}
   \ELSE
   \STATE $\tilde k^t=-1$ \hfill\texttt{:Case 3:}
   \ENDIF
   \STATE $x_{i^t}^{t+1}=x_{i^t}^{t}-\alpha(\nabla_{i^t}f(x^{t})+\tilde k^t\tilde\nabla_{i^t}G_F(x^t))$,
   $x_{i}^{t+1}=x_{i}^{t}$,\quad  if \quad $i\neq i^t$
   \ENDFOR
\end{algorithmic}
\end{algorithm}
% \vspace{-1.5cm}
% \end{minipage}
% \end{wrapfigure}
\begin{shadowboxtext}
\begin{theorem}\label{convergence_practical}
For an $n$-sided $\mu$-PL function $f(x)$ satisfying \cref{L_Lip}, by implementing \cref{arbcd_practical} with $\alpha$ be small enough, $\beta\leq\frac{1}{L}$ and $T'\geq C'\log\big(\frac{1}{\gamma\alpha}\big)/\log(\frac{1}{1-\mu\beta})$ where $C'$ only depends on the function parameters, 

\begin{itemize}[leftmargin=7pt]
\item in Case 1, we have
\begin{small}
$
\mathbb{E}[f(x^{t+1})-G_F(x^{t+1})|x^t]\leq (1-\frac{\mu\alpha(1-\gamma)}{2})(f(x^t)-G_F(x^t)),
$
\end{small}

\item in Case 2, we have
\begin{small}
$
    \mathbb{E}[f(x^{t+1})-G_F(x^{t+1})|x^t]\leq \big(1-\frac{(L+L')\mu\alpha^2}{4}\big)\ (f(x^t)-G_F(x^t)),
$
\end{small}

\item in Case 3, we have  $f\!-\!G_F$ be non-increasing. Furthermore, if $f\!-\!G_F$ satisfies $(\theta,\nu)$-PL condition and case 3 occurs from iterates $t$ to $t+k$, then
\begin{small}
\begin{equation*}
    \mathbb{E}[f(x^{t+k})-G_F(x^{t+k})|x^t]=\mathcal{O}\Big(\frac{f(x^{t})-G_F(x^{t})}{k^{\frac{\theta}{2-\theta}}}\Big). 
\end{equation*}
\end{small}
\end{itemize}
\end{theorem}
\end{shadowboxtext}


%\begin{algorithm}[tb]
%   \caption{Adaptive randomized Block Coordinate Descent (A-RBCD)}
%\begin{algorithmic}\label{arbcd_practical}
%   \STATE {\bfseries Input:} initial point $x^0=(x_1^0,...,x_n^0)$, positive number $\{\alpha_t\}$, $\beta$, $C$ and $\gamma<1$
%   \FOR{$t=0$ {\bfseries to} $T-1$}
%   \STATE sample $i^t$ uniformly from $\{1,2,...,n\}$
%   \FOR{$j=1,...,n$}
%   \STATE $y_j^{t,0}=x_{j}^{t}$
%   \FOR{$t_i=0,...,T'-1$}
%   \STATE $y_j^{t,t_i+1}=y_j^{t,t_i}-\beta\nabla_{j}f(y_j^{t,t_i},x_{-j}^{t})$
%   \ENDFOR
%   \ENDFOR
%   \STATE compute $\tilde\nabla G_F(x^t):=\frac{1}{n}\sum_{l=1}^n\nabla f(y_l^{t,T'},x_{-l}^{t})$
%   \IF{$\langle\tilde\nabla G_F(x^t),\nabla f(x^t)\rangle\leq (\gamma-\gamma\frac{\alpha_t^{3}}{13}) \|\nabla f(x^t)\|^2$}
%   \STATE $\tilde k^t=0$ \hfill\texttt{:Case 1:}
%   \ELSIF{$\frac{(\|\tilde\nabla G_F(x^t)\|^2-\langle\nabla f(x^t),\tilde\nabla G_F(x^t)\rangle)^2}{\|\tilde\nabla G_F(x^t)\|^4}>C$ and $\langle\tilde\nabla G_F(x^t),\nabla f(x^t)\rangle\geq (\gamma-\gamma\frac{\alpha_t^{3}}{13}) \|\nabla f(x^t)\|^2$ {\color{blue} This should hold as it is in the elseif!?}}
%   \STATE $\tilde k^t=-1+\frac{\langle\nabla f(x^t),\tilde\nabla G_F(x^t)\rangle-\|\tilde\nabla G(x^t)\|^2}{\|\tilde\nabla G_F(x^t)\|^2}$\hfill\texttt{:Case 2:}
%   \ELSE
%   \STATE $\tilde k^t=-1$ \hfill\texttt{:Case 3:}
%   \ENDIF
%   \STATE $x_{i^t}^{t+1}=x_{i^t}^{t}-\alpha_t(\nabla_{i^t}f(x^{t})+\tilde k^t\tilde\nabla_{i^t}G_F(x^t)), \quad x_{i}^{t+1}=x_{i}^{t}$, if $i\neq i^t$
%   \ENDFOR
%   \STATE {\bfseries Output:} $x^{T}=(x_1^{T},...,x_n^{T})$
%\end{algorithmic}
%\end{algorithm}






==> neurips_2025/7_applications.tex <==
% \vspace{-.3cm}
\section{Applications}\label{sec:applications}

% \textcolor{red}{The thing I am still not sure is, if we put two experiments that doesn't have good improvement on the result, will the reviewers criticize on this? How should we convince them?}
% \textcolor{blue}{
% That is true. One thing is to emphasize that your alg does not need boundedness while BCD needs it for having a guarantee. Another is to look for examples in which your algo is faster. For example, if you run your alg for the function $f_1$ in Fig 2. would your algorithm show linear convergence?
% If the function is bounded then our algs should perform similar to the BCD, right?
% What other scenario, you expect that your alg perform better?
% }
In this section and in Appendix \ref{sec:add_app}, we study well-known nonconvex problems that satisfy the $n$-sided PL condition, as well as scenarios where A-RBCD converges while BCD and Adam optimizer \cite{kingma2015adam} fail to do so.



\textbf{Function with only strict saddle point: } We consider the function $f(x,y)=(x-1)^2+4(x+0.1\cos(x))y+(y+0.1\sin(y))^2$. The problem aims at finding the NE $(x^\star,y^\star)$, 
\begin{equation*}
\begin{aligned}
    f(x^\star,y^\star)\leq f(x,y^\star),\forall x,\quad     f(x^\star,y^\star)\leq f(x^\star,y),\forall y.    
\end{aligned}
\end{equation*}
% \begin{figure}
% \centering
% \subfigure[]{
% \includegraphics[width=0.47\linewidth,height=2.8cm]{neurips_2025/game_allocation.png}}
% \subfigure[]{
% \includegraphics[width=0.47\linewidth,height=2.5cm]{neurips_2025/strict_saddle_allocation.png}}
% \caption{(a) Performances of A-RBCD, BCD, and Adam on function $c_A+c_B$ shown in (b).}\label{fig:game_allocation}
% \vspace{-.3cm}
% \end{figure}
Figure \ref{fig:non_convergence} represents the convergence results of A-RBCD and BCD with 100 random initializations. The iterates of A-RBCD always converge to the NE at a linear rate, while BCD diverges. Note that the NE is a strict saddle point.  

\textbf{Competitive Resource Allocation Game:}
Consider a two-player game where two companies, A and B, are competing for resources. In this case, they are both trying to minimize their cost of using the resource, denoted by $x_A$ and $x_B$, but the cost depends on how much of the resource each company uses \citet{roughgarden2009algorithmic}. 
Let us assume the following quadratic cost functions: $c_A(x_A,x_B)=x_A^2-2x_A x_B$ and $c_B(x_A,x_B)=x_B^2-2x_A x_B$.
The quadratic terms represent the individual costs of using the resources and the multiplicative term indicates the interaction cost between the two companies. Total costs of this game is $c_A(x_A,x_B)+c_B(x_A,x_B)$.
It is straightforward to see that this objective is 2-sided PL but is not lower bounded. The only NE point is $(0,0)$, which is a strict saddle point. 
Figure \ref{fig:non_convergence} shows the convergence results of A-RBCD and BCD with 100 random initializations. The iterates of A-RBCD always converge to the NE at a linear rate, while BCD diverges. 




% \textbf{Linear Residual Network: } It aims to learn the linear transformation $R:\mathbb{R}^d \rightarrow\mathbb{R}^d$, such that $y=Rx+\xi$, where $\xi\sim \mathcal{N}(0,I_d)$ and $I_d$ denotes the identity matrix of dimension $d$. The learned model can be parameterized by a sequence of weight matrices $A_1,..., A_n\in\mathbb{R}^{d\times d}$, such that
% $h_0=x$, $h_j=(I+A_j)h_{j-1}$, $\hat{y}=h_n$. 
% Thus, the objective function of this problem is given by
% \begin{equation*}
% \begin{aligned}
%         f(A_1,...,A_n):&=\mathbb{E}[\|\hat{y}-y\|^2]=\mathbb{E}\big[\|(I+A_n)...(I+A_1)x-Rx-\xi\|^2\big].
% \end{aligned}
% \end{equation*}
% Even though $(I+A_n)\cdots(I+A_1)$ is a linear map, the optimization problem on the factored variables $(A_1,..., A_n)$ is nonconvex \citep{hardt2016identity}. %{As we have shown in \cref{proof:LRN_convergence}, this function satisfies both the $n$-sided PL condition if $\max_i\|A_i\|<1$, and Assumption \ref{ass:new}. Thus, linear convergence can be achieved using both random BCD and A-RBCD. We also demonstrated this through empirical evidence.}
% More precisely, we considered two settings: (1) $d=3, n=5$ and (2) $d=5, n=10$ with covariance matrices $\Sigma=\mathbb{E}[xx^T]=I_d$, and applied the A-RBCD algorithm to both settings. 
% Figure \ref{fig:exp1} illustrates the resulting error curves on a log-scaled y-axis, obtained from 100 trials. Each trial is obtained by randomly selecting the diagonals of matrix $R$ according to $U(0.5,1.5)$ and initializing $A_i$s with random entries according to $U(-0.1,0.1)$. 
% \begin{figure}
% \centering  
% \subfigure[$n=5, d=3$]{
% \includegraphics[width=0.47\linewidth,height=2.8cm]{5_LRN.png}}
% \subfigure[$n=10, d=5$]{
% \includegraphics[width=0.47\linewidth,height=2.8cm]{10_LRN.png}}
% \caption{Performance of the A-RBCD and RBCD on linear residual network problems for different network sizes illustrates linear convergence, as advocated by \cref{convergence_ideal_kt0}.}\label{fig:exp1}
% \vspace{-.3cm}
% \end{figure}

% \vspace{-.1cm}
\textbf{Infinite Horizon $n$-player Linear-quadratic (LQR) Game:} 
The objective function is 
\begin{small}
\begin{equation*}
    \mathbb{E}_{x_0\sim\mathcal{D}}\big[\sum_{t=0}^{+\infty}[(x^t)^T Q x^t+\sum_{i=1}^n ((u_i^t)^T R_i u_i^t]\big],
\end{equation*}
\end{small}
where $x_t$ denotes the state, $u_i^t$ is the input of $i$-th player at time $t$, and $i\in[n]$. The state transition of the system is characterized by 
$x^{t+1}=Ax^t+\sum_{i=1}^n B_iu_i^t$, where $A\in\mathbb R^{k\times k}$ and $B\in\mathbb R^{k\times d}$.
When players apply linear feedback strategy, i.e., $u_i^t=-K_i x^t,$, the objective function becomes 
\begin{small}
\begin{equation*}
    f(K_i,K_{-i})=\mathbb{E}_{x_0\sim\mathcal{D}}\big[\sum_{t=0}^{+\infty}[(x^t)^T Q x^t+\sum_{i=1}^n ((K_ix_i^t)^T R_i K_ix_i^t]\big].
\end{equation*}
\end{small}
If $K_i$s are bounded and $\Sigma_0=\mathbb{E}_{x^0\sim\mathcal{D}}[x^0(x^0)^T]$ is full rank, the objective function $f$ satisfies the $n$-sided PL condition (see  \cref{proof_n_sided_LQR} for a proof). 
However, as it is discussed in \cite{fazel2018global}, even the objective of one-player LQR is not convex. Subsequently, the objective function of the $n$-player LQR game is not multi-convex. See \cref{ce_LQR_convex} for examples. Fig. \ref{fig:lqr} demonstrates the resulting error curve, $f(K^t)\!-\!G_f(K^t)$, and $\rho\!:=\!\frac{\langle\nabla f(K^t),\nabla G_f(K^t)\rangle}{\|\nabla f(K^t)\|^2}$. This shows that during the updating procedure, the third case did not occur. 
\begin{figure}
\centering
\subfigure[]{
\includegraphics[width=0.4\linewidth,height=3cm]{non_convergence.png}}
\subfigure[]{
\includegraphics[width=0.4\linewidth,height=3cm]{neurips_2025/game_allocation.png}}
\caption{(a) Performances of A-RBCD, BCD, and Adam on function $f(x,y)$ (b) Performances of A-RBCD, BCD, and Adam on function $c_A+c_B$.}\label{fig:non_convergence}
\end{figure}
\begin{figure}
\centering
% \subfigure[\footnotesize{$n=5$,\ $d=3$}]{
% \includegraphics[width=0.47\linewidth,height=2.8cm]{5.png}}
\subfigure[\footnotesize{Convergence when $n=10$,\ $d=5$}]{
\includegraphics[width=0.4\linewidth,height=2.8cm]{10.png}}
% \subfigure[\footnotesize{$n=20$,\ $d=10$}]{
% \includegraphics[width=0.47\linewidth,height=2.8cm]{20.png}}
\subfigure[\footnotesize{$\rho$}]{
\includegraphics[width=0.4\linewidth,height=2.8cm]{rho.png}}
\caption{(a)Performance of the A-RBCD and RBCD on LQR game. The y-axis is on the log scale.(b)Value of $\rho$ during the iterations.}\label{fig:lqr}
\vspace{-.3cm}
\end{figure}

\textcolor{blue}{
- $x^TAx+b^Tx$\\
- Congestion Games\\
- Games on Graph 
}

==> neurips_2025/8_conclusion.tex <==
\vspace{-.2cm}
\section{Conclusion}
\vspace{-.1cm}
In this paper, we identified a subclass of nonconvex functions called $n$-sided PL functions and studied the convergence of GD-based algorithms, particularly the BCD algorithm, for finding their NEs. The $n$-sided PL condition is a reasonable extension of the gradient dominance condition, which holds in various problems. 
We showed that the convergence rate of such first-order algorithms in this subclass of functions depends on a local relation between the function $f$ and the average of the best responses $G_f$. Subsequently, we proposed two novel algorithms, IA-RBCD and A-RBCD, equipped with $G_f$, that provably converge to the NE set almost surely with random initialization, even if the function is not lower bounded and has strict saddle points. We hope this work can shed some light on the understanding of nonconvex optimization.





%In this paper, we identify a subclass of nonconvex problems with block structure, represented by the so-called $n$-sided PL condition. We also propose the first two random algorithms, IA-RBCD and A-RBCD that provably converge to the Nash Equilibrium in most of cases, while protect the privacy of every blocks. We hope this work can shed some light on the understanding of nonconvex optimization, especially the PL condition: (1) the $n$-sided PL condition is a reasonable extension for the strong PL condition, with the existence of average of best response function $G_f$; (2) the complexity of solving a nonconvex optimization problem may depends on the relation between the function $f$ and average of best response $G_f$; It remains interesting to explore whether applying similar algorithm can result in linear convergence rate to the Nash Equilibrium or even the global minimum.

==> neurips_2025/limitations.tex <==
\section{Limitations}

==> new_result.tex <==
In order to find the Nash Equilibrium, the normal block coordinate descent requires \cref{lower-bounded}, i.e. the function value is lower-bounded. However, this is impossible for a large class of function. For example, the quadratic function $f(x)=x^TAx$ with $\lambda_{min}(A)<0$ is not lower bounded, and has one saddle point at zero. \cite{lee2016gradient} proved that gradient descent doesn't converge to the saddle point almost surely with random initialization. While \cref{arbcd_ideal} and \cref{arbcd_practical}, the lower-bounded function value is not a requirement. As long as the norm of derivative $\|\nabla f(x)\|$ is coercive as $\|x\|$ goes to infinity, the iterates is bounded and converge to the NE set. If further case 1 and case 2 in the \cref{arbcd_ideal} and \cref{arbcd_practical} are always satisfied as time is large enough, it converge to a point in the NE set.
